UI-Venus-2 Technical Report

Multimodal GUI agents have emerged as a promising paradigm for digital task automation, yet transitioning from benchmark-oriented models to dependable real-world applications remains challenging due to limited environment coverage, brittle task construction, and unreliable reward verification. In this work, we present UI-Venus-2, a general-purpose foundation GUI agent designed to operate across mobile, web, and desktop environments through a unified closed-loop reasoning-action framework. To bridge the gap toward practical deployment, we jointly scale three critical dimensions: (1) Environments, expanding coverage to more than 170 multilingual mobile apps and native desktop operating systems; (2) Tasks, employing a deep-research pipeline for function-grounded instruction generation; and (3) Verification, adopting trace-level and sample-level evaluators with visual keypoints and multi-model voting to ensure reliable RL signals for training. Furthermore, we integrate safety-aware mechanisms to ensure controlled execution of consequential actions. By offering a capable, efficient, and open-source foundation, UI-Venus-2 advances the field toward more generalizable, verifiable, and self-reflective agents for real-world applications.

==> doc/daas.tex <==
\subsubsection{Device as a Service (DaaS)}\label{sec:daas}

% Training and deploying a GUI Agent that can generalize across heterogeneous devices imposes stringent requirements on the underlying execution environment in terms of uniformity, extensibility, and performance. Unlike simulators tailored to a single device category, such an environment must support a wide range of heterogeneous device types, provide a unified abstraction over diverse interaction protocols, and, under strict network-isolation policies, securely and efficiently expose large-scale device resources to upstream training and deployment frameworks.

Training and deploying a GUI Agent capable of generalizing across heterogeneous devices imposes stringent demands on the underlying execution environment in terms of uniformity, extensibility, and performance. Unlike simulators designed for a single device category, such an environment must accommodate a wide variety of device types, offer a unified abstraction over diverse interaction protocols, and—under strict network-isolation policies, securely and efficiently expose large-scale device resources to upstream training and deployment frameworks. Therefore, we build a unified Device-as-a-Service (DaaS) layer (Figure~\ref{fig:daas_framework}) to meet these requirements. It consists of two core components: the Group Control Gateway (GCGW) and the Unified Client SDK, whose design and implementation are detailed next.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/daas.pdf}
\caption{\textbf{Architecture of the Unified Device-as-a-Service (DaaS) layer.} This framework bridges upstream tasks (Training and Inference) with downstream heterogeneous device clusters (Chrome, Mobile, and Desktop). The Multi-language DaaS SDK provides a unified abstraction for diverse interaction protocols, while the Group Control Gateway (GCGW) ensures high-performance and secure resource exposure through secondary hash routing, zero-copy I/O, and a multi-protocol reverse proxy.}
\label{fig:daas_framework}
\end{figure}
% To address these challenges, we design and implement a unified Device-as-a-Service (DaaS) layer, centered on a high-performance Group Control Gateway (GCGW) for large-scale device orchestration. The gateway abstracts and consolidates heterogeneous control protocols across diverse devices (e.g., Android, Chrome, and Linux containers), and exposes efficient, transparent access through a single ingress {\color{red}(ports 80/443) mask ip}. Leveraging intelligent routing and a highly concurrent execution model, the system sustains large-scale, high-throughput workloads with millions of device-operation requests per day. In the following, we detail the key design components of our DaaS layer.
% To address these challenges, we designed a unified Device-as-a-Service (DaaS) layer. Its core is a high-performance Group Control Gateway (GCGW) for large-scale device orchestration, which abstracts heterogeneous control protocols across diverse platforms (\emph{e.g.}, Android, Chrome, and Linux containers). The gateway provides efficient, transparent access through a unified ingress. Thus, the system is capable of sustaining high-throughput workloads at scale. The following sections detail the key design components of our DaaS layer.
% To address the challenges of large-scale device orchestration and protocol heterogeneity across diverse platforms, we designed a unified Device-as-a-Service (DaaS) layer as shown in Figure~\ref{fig:daas_framework}. The DaaS layer is primarily composed of two core components: the Group Control Gateway (GCGW) and the Unified Client SDK. The following sections detail the design and implementation of these two components.

% Therefore, we build a unified Device-as-a-Service (DaaS) layer (Figure~\ref{fig:daas_framework}) to meet these requirements. It consists of two core components: the Group Control Gateway (GCGW) and the Unified Client SDK, whose design and implementation are detailed next.

% \textbf{Group Control Gateway (GCCW). }We have built a unified Group Control Gateway (GCGW). Acting as a reverse proxy, the gateway centrally receives all device-operation requests over the fixed and selected ports and securely forwards them to thousands of individual devices deployed within the VPC network, including Android devices, Chrome browsers, and desktop machines. 
% Our device pool comprises multiple device types (e.g., Android devices and Chrome browsers), whose native control protocols (e.g., ADB and CDP) differ and expose incompatible ports and APIs. GCGW is designed around ``protocol'' as the core abstraction, enabling extensible support for heterogeneous device types. To date, we have implemented several protocol plugins, including androidv1 (an ADB wrapper), cdpv1 (Chrome DevTools Protocol), playwrightv1 (a streamlined browser automation interface), and sshShellv1.

% \textbf{Group Control Gateway (GCGW):} We designed and implemented a unified Group Control Gateway (GCGW) to serve as a centralized reverse proxy. It receives all device-operation requests through designated ports and securely routes them to thousands of individual devices within the VPC network—including Android devices, Chrome browsers, and desktop machines. Specifically, our device pool consists of multiple device types (\emph{e.g.}, Android devices and Chrome browsers), each with distinct native control protocols (such as ADB and CDP) that expose incompatible ports and APIs. The GCGW is designed around a protocol-centric abstraction, enabling extensible support for heterogeneous devices. Currently implemented protocol plugins include: androidv1 (an ADB wrapper), cdpv1 (Chrome DevTools Protocol), playwrightv1 (a streamlined browser automation interface), and sshShellv1.

% \textbf{Optimized Routing for Stateful Connections:} Protocols such as ADB and CDP are inherently stateful and rely on long-lived connections. Adopting a purely randomized load-balancing strategy in the GCGW cluster would lead to the classic $M\times N$ connection explosion problem—over time, $M$ gateway nodes could each establish connections to all $N$ devices, rapidly exhausting connection resources and rendering gateways unavailable. To address this, we innovatively employ an internal secondary hash routing algorithm. This ensures that all connection requests targeting a specific device are consistently routed to the same fixed node within the GCGW cluster, completely eliminating the connection explosion issue. %This solution reduces the number of persistent device connections maintained per GCGW node from over 300 to fewer than 20, representing a qualitative improvement in resource utilization.

% \textbf{Efficient Internal Forwarding Mechanism:} The aforementioned routing strategy necessarily involves secondary forwarding of certain requests between internal nodes in the GCGW cluster. To minimize forwarding overhead, we extensively employ streaming transmission and zero-copy I/O technologies in intra-gateway communications. This ensures that request chains requiring internal forwarding exhibit virtually no additional latency or throughput degradation compared to direct connections.

% \textbf{High-Concurrency Coroutine Model:} Typical device operation scenarios are characterized by high concurrency but relatively low request frequency per individual connection. To handle massive connection volumes, the GCGW gateway adopts a comprehensive coroutine-based concurrency model for both underlying communication and business logic processing. This design enables the system to theoretically maintain hundreds of thousands of concurrent connections with minimal memory overhead, perfectly matching the "high-concurrency, low-frequency" access pattern of the device pool.

\textbf{Group Control Gateway (GCGW).} The GCGW serves as a high-performance centralized reverse proxy and the orchestration core of the DaaS layer. It abstracts heterogeneous control protocols across diverse platforms—including Android (ADB), Chrome (CDP), and Linux containers (SSH)—enabling extensible support through a protocol-centric abstraction.

To ensure system stability and performance under high-throughput workloads, the GCGW integrates several key architectural optimizations. First, to handle stateful protocols like ADB and CDP which rely on long-lived connections, the GCGW employs an internal secondary hash routing algorithm. This mechanism ensures that all requests for a specific device are consistently routed to the same gateway node, effectively preventing the ``$M\times N$ connection explosion'' problem($M$ gateway nodes and $N$ devices) and significantly reducing the connection overhead per node. To support this routing strategy without sacrificing performance, the gateway utilizes streaming transmission and zero-copy I/O for internal forwarding between nodes, ensuring near-zero additional latency. Furthermore, the entire GCGW architecture is built on a high-concurrency coroutine model. This design is specifically tailored for the ``high-concurrency, low-frequency'' access patterns of device operations, allowing the system to maintain hundreds of thousands of concurrent connections with minimal memory overhead.

% \textbf{Unified Client SDK:} Although GCGW unifies access to all devices through one port, requiring users to manually handle gateway authentication, protocol selection, and device lifecycle management (preemption, heartbeat, and release) would still be cumbersome. To address this, we developed a multi-language DaaS SDK. This SDK encapsulates device resource management, security authentication, and semantic interactions with all internal protocols supported by GCGW behind an intuitive API, significantly reducing integration costs for downstream users.

% \textbf{Unified Client SDK.} While the GCGW provides a unified ingress for device access, a Unified Client SDK was developed to further shield downstream users from the complexities of infrastructure management. The multi-language SDK provides a high-level API that encapsulates several critical functions. Specifically, the SDK automates device lifecycle management—including preemption, heartbeats, and release processes—while simultaneously streamlining security and authentication through simplified gateway access and secure token management. Furthermore, it facilitates semantic interaction by offering a unified interface for various internal protocols supported by the GCGW, such as androidv1, cdpv1, playwrightv1, and sshShellv1. By abstracting these low-level operations, the SDK significantly reduces integration costs and enables developers to prioritize business logic over protocol-specific nuances.

\textbf{Unified Client SDK.} To further shield downstream users from the complexities of infrastructure management, a multi-language Unified Client SDK was developed that acts as a high-level API layer atop the GCGW. This SDK encapsulates several critical functions into a streamlined workflow. Specifically, it automates device lifecycle management, including device preemption, heartbeat maintenance, and resource release. 
% For security, the SDK simplifies the authentication process and manages access tokens transparently. 
Furthermore, it provides a unified semantic interaction interface that standardizes communication across various internal protocols. 
% By abstracting these low-level operations, the SDK significantly lowers integration barriers, enabling developers to focus on higher-level business logic rather than protocol-specific technicalities.
By abstracting these low-level operations, the SDK significantly lowers integration barriers, allowing downstream teams to concentrate on building and operating the end-to-end training pipeline for large-scale online reinforcement learning of GUI-specialized models, as well as the production deployment of those GUI-focused models—rather than dealing with protocol-specific technicalities.

% Through the implementation of these technical solutions, our DaaS layer now stably supports the following scale and performance indicators:
% \begin{itemize}
%     \item \textbf{Scale and Throughput.} The system successfully integrates thousands of heterogeneous devices, forming a stable service architecture handling millions of operation requests daily.
%     \item \textbf{Operational Latency.} End-to-end latency for individual device operations is maintained under one second, satisfying real-time requirements for interactive applications.
%     \item \textbf{Resource Allocation Efficiency:} Device resource allocation and scheduling achieve millisecond-level responsiveness, enabling rapid elastic provisioning.
%     \item \textbf{High-Concurrency Support.} The system has successfully supported over thousands concurrent reinforcement learning training tasks, handling millions of API calls daily, validating its exceptional stability and scalability under high-load scenarios.
% \end{itemize}

% In summary, our DaaS layer is not merely a simple device exposure service, but a comprehensive solution deeply integrating protocol abstraction, intelligent routing, high-performance communication, and multi-language SDKs. While ensuring security and manageability, it transforms heterogeneous, distributed device resources into standardized, easily accessible, and massively scalable service capabilities, providing a robust and reliable device infrastructure foundation for upstream applications such as agent training and automated testing.

By implementing these architectural optimizations, the DaaS layer achieves the following performance benchmarks:
\begin{itemize}
    \item \textbf{Scale and Throughput:} The system successfully integrates thousands of heterogeneous devices, establishing a resilient architecture that processes millions of operation requests daily.
    \item \textbf{Resource Allocation Efficiency:} Device resource allocation and scheduling achieve millisecond-level responsiveness, enabling rapid elastic provisioning.
    \item \textbf{High-Concurrency Support:} The system has successfully supported large-scale reinforcement learning training tasks involving hundreds to thousands of concurrent devices, which demonstrated superior stability and extensibility under high-load conditions.
\end{itemize}

% In conclusion, the DaaS layer transcends simple device exposure by providing a sophisticated orchestration solution that integrates protocol abstraction, intelligent routing, and high-performance communication. By transforming fragmented, heterogeneous device resources into standardized and scalable service capabilities, it provides a reliable foundation for diverse upstream applications such as large-scale agent training, automated testing and automated data annotation.

==> doc/data.tex <==
\section{Data Preparing}

\subsection{Data Collection}



The pipeline constructs GUI-agent training data from a real application and then grows that data through a flywheel. A document-driven pass produces the first batch of instructions, trajectories, and verifiers. Later rounds no longer start from the document. They reverse-synthesize new instructions from existing trajectories, collect new rollouts, and feed the cleaned data back into reverse synthesis.
\paragraph{Cold-start collection.}
We first obtain an application together with its documentation and perform deep research over the documentation to systematically recover the application's functional capabilities, page structure, and the mapping between interface elements and executable actions. The research process further synthesizes these capabilities into feasible multi-step user workflows, which serve as the basis for seed instruction generation.

Based on this structured knowledge, an instruction writer generates candidate instructions that correspond to real and executable application functions. Each candidate is subsequently evaluated by an independent LLM judge from a different model family, which verifies its executability, unambiguity, and fidelity to the documented functionality. Accepted instructions are added to the instruction pool and used by an agent to collect execution trajectories. Finally, we apply a lightweight cleaning process to the collected trajectories to obtain the initial training set. This document-driven process is performed only once to cold-start our training data generation flywheel.

% \textcolor{red}{\@ suyu  implement deep research}
% We first obtain the application and its documentation, then run a deep search over the document to recover the function set, the page inventory, and the mapping from controls to actions. 

% After that,
% an instruction writer generate candidate instructions based on the knowledge from the deep research phase. Each candidate is then reviewed by an instruction judge from a different LLM family, which checks executability, unambiguity, and fidelity to a real function. Accepted instructions enter our instruction pool.
% An agent then collects trajectories from this pool, and a light cleaning pass turns those trajectories into the seed training set. This pass is run once and only to cold start our training data generation flywheel.


\paragraph{Reverse instruction synthesis.}
Once the seed training set is available, later rounds generate instructions
from collected trajectories. The instruction writer receives a trajectory fragment,
including several screenshots and their neighboring actions, and infers an instruction
that could potentially have produced the observed behavior. The instruction judge then
applies the same criteria used during cold-start collection, checking that the
instruction is executable, unambiguous, and grounded in a real application
function. Valid candidates are compared against the current instruction pool.
Overly similar are removed, while instructions that introduce a new goal,
control, or action sequence are retained. This process recovers
executable tasks that are absent or underspecified in the documentation, and
therefore extends the cold-start instruction pool beyond what can be obtained
from documents alone.

\paragraph{Data flywheel.}
Each retained instruction is added to the instruction pool and used by the
agent to collect a new trajectory. After a light cleaning process, the trajectory is
merged into the training set and becomes a source for the next round of
reverse instruction synthesis. Another round therefore starts with the
current training data, produces new instructions from trajectory fragments,
filters them through the instruction judge, and collects new trajectories from
the accepted instructions. Repeating this process grows the training set while
exposing screenshots and action sequences that were absent from earlier
rounds.

\paragraph{Paired verifiers.}
\textcolor{red}{fangbie gogogo}
Each instruction is generated together with a success verifier. When task
completion can be read from application or system state, we use a Python
assertion to check the result directly. This applies, for example, to creating
or deleting a document, modifying its content or format, or changing the
system volume. For tasks whose outcomes cannot be reliably inspected through
code, such as image editing, the instruction includes an explicit success
criterion that can later be checked against the collected trajectory by an
LLM judge.

\paragraph{Two judge roles.}
The instruction judge and the trajectory judge serve different purposes.
Before trajectory collection, the instruction judge sees only the candidate
instruction and decides whether it defines a valid task. After collection, the
trajectory judge sees both the instruction and the resulting trajectory and
determines whether the task was completed. The trajectory judge is used only
when a Python verifier is unavailable. Thus, the first judge controls which
instructions enter the collection pipeline, while the second evaluates the
outcome of the collected behavior.


\noindent\textbf{Mobile}
We collect data from more than 200 real-world Chinese and English android applications. For Chinese applications, we build an in-house collection platform using physical Android phones; for English applications, we collect data in Android emulators.

Because LLMs lack prior knowledge of an application's capabilities, direct task generation often hallucinates unsupported functions. We therefore construct an application-specific \emph{function tree} and condition task generation on it, improving both validity and diversity. The tree is built in two stages: (1) we extract an initial hierarchy of functions from deep-research reports and AI-generated answers grounded in community sources, establishing a functional prior for the application; and (2) after collecting initial tasks and screenshots, we apply semantic recognition and function aggregation to discover and consolidate observed capabilities, iteratively enriching the tree for subsequent task generation.

\noindent\textbf{Browser}
We construct a diverse pool of browser tasks with broad domain coverage and substantial interaction complexity. To build the domain pool, we curate websites from diverse public web sources, including established browser-agent resources and the Tranco ranking \cite{pochat2018tranco}. We first remove inaccessible websites through automated crawling. For the remaining candidates, we feed their homepage HTML to Kimi 2.6 to assess each website along four dimensions: dynamicity, interactivity, content richness, and visual quality, retaining websites that provide rich and diverse interaction opportunities. This process yields over 4,000 high-quality domains, which are further organized into 19 website categories, such as e-commerce, travel, education, finance, and healthcare.

% Based on this domain pool, we generate tasks by combining realistic user scenarios with different task objectives. Specifically, we define 10 scenarios that reflect common real-world needs, such as planning a vacation, preparing for a move, or researching a major purchase, and pair them with five task types: Planning, Comparison, Research, Shopping, and Booking. For each combination, we select 2--4 websites from relevant domain categories and generate a task that requires coordinated interactions across these websites, resulting in complex multi-step and cross-site trajectories.

As illustrated in Fig.~\ref{fig:venus20_overview}, we follow a deep-research-based task generation pipeline to construct diverse browser tasks from the curated domain pool. In addition, we leverage tasks from InSTA-150k-v3 \cite{Trabucco2025InSTA}, where each task is annotated with task-specific success criteria. We use the number of criteria as a proxy for task complexity, rank the tasks accordingly, and select 45K relatively challenging tasks for data collection.

Trajectories are collected in a Playwright-based browser environment that provides 15 browser actions, such as clicking, scrolling, typing, dragging, and hovering. During collection, the agent operates in a closed loop: it observes the current screenshot and interaction history, predicts the next action, executes it in the browser, and continues with the updated observation. To improve the robustness of large-scale collection on real-world websites, requests are distributed across domains and executed with real Chrome sessions, while domains that remain inaccessible are discarded

We apply both trajectory-level and step-level filtering to improve data quality. At the trajectory level, GPT-5 mini together with the WebVoyager judge prompt is used to evaluate task completion from the full interaction history, and only successful trajectories are retained. At the step level, rule-based filters remove redundant or ineffective behaviors, including repeated waits or clicks, opposite-direction scrolling, and cyclic action patterns such as ABAB or ABCABC. Importantly, we do not remove all erroneous actions from successful trajectories. When the agent deviates from the intended path but subsequently recovers, the erroneous steps are retained in the interaction history, allowing the model to learn corrective actions conditioned on realistic error states and thereby improving its error-recovery capability.

\noindent\textbf{Computer}

\noindent\textbf{Grounding}
Our grounding data are constructed through a unified programmatic synthesis framework that tightly couples executable interface code, rendered visual appearance, and semantic supervision. Starting from diverse natural-language task scenarios, optionally augmented with user personas and reference screenshots, a code-capable model generates executable HTML/CSS/JavaScript interfaces that jointly encode layout, textual content, interactive components, and stateful behaviors \cite{yang2025scaling}. The generated interfaces are then rendered in a controlled browser environment, where screenshots, DOM structure, element states, and geometry are captured in a single pass, ensuring intrinsic alignment between visual observations and their underlying semantic organization. Candidate interactive elements are subsequently identified through a combination of DOM semantics, accessibility cues, and interaction-related signals, and are annotated with precise bounding boxes, target coordinates, visible text, ARIA attributes, and contextual information. To ensure that annotations correspond to genuinely actionable regions, the pipeline further applies explicit visibility, occlusion, and painted-pixel reasoning, including viewport clipping, scroll containment, nine-point hit testing, and text-node-level refinement. Finally, the verified elements are transformed into grounding supervision by generating multiple linguistically diverse intents for each target, incorporating both valid instructions and infeasible cases as hard negatives, and exporting the same interface into multiple training formats such as point grounding, bounding-box prediction, SFT-based instruction grounding, and RL-oriented samples. This design enables scalable construction of richly annotated grounding data with fine-grained alignment among interface appearance, semantic meaning, interaction state, and pixel-level target localization. We provided some synthetic data samples (see Reference Image 1).

\noindent\textbf{CAPTCHA}
We develop a four-stage programmatic pipeline that transforms explicitly verified CAPTCHA puzzle states into realistic mobile-style interfaces and automatically derives pixel-aligned, semantically rich supervision for GUI agents. The pipeline begins with \textbf{verified puzzle synthesis}, where type-specific rule engines instantiate solvable challenges across 70 CAPTCHA types by combining constraint-based generation with diverse visual assets; critically, each puzzle is represented as a machine-checkable latent state that serves as the single source of truth for its rendered content, target geometry, executable actions, and reasoning traces. This design enables automatic verification of solution validity, controlled difficulty and diversity, multi-solution expansion, and the generation of both direct and reflective reasoning trajectories without manual annotation. The verified content is then passed to an independent \textbf{interface rendering} stage, which wraps the puzzle into realistic mobile CAPTCHA layouts and webpage contexts while deterministically remapping all geometric annotations to the final canvas, thereby separating semantic correctness from visual presentation and allowing interface realism to be improved without affecting the underlying supervision. Finally, the \textbf{agent-ready export} stage converts the annotations into a unified GUI-agent action space and resolution-independent coordinate representation, and automatically produces both SFT- and RL-oriented training formats containing reasoning, normalized geometry, and executable action sequences. Overall, the pipeline establishes a deterministic correspondence among \textbf{puzzle logic, rendered pixels, spatial annotations, actions, and reasoning}, enabling large-scale synthesis with no per-sample manual labeling while simultaneously providing strong guarantees of annotation correctness, controllable data diversity, realistic interface distributions, and flexible support for downstream agent training.

% \subsection{Data Generation Loop}

% %\noindent\textbf{Iterative Data Refinement (IDR):} 

% %\noindent\textbf{Self-Evolving Feedback via Real-Device Execution:} 
% % To improve robustness of model in real-world environments, we developed a Self-Evolving data generation pipeline based on our DaaS system(refer to Section~\ref{sec:daas}). As shown in Figure~\ref{fig:daas_feedback}, we first set the seeds for task generation via an open-source MLLM to get a large number of candidate task prompts. Following a semantic verification based on the prompt embedding's similarity, the checked and unique task prompts are stored in the task bank and sent to the DaaS environment for further interaction with UI Agents, which executes the prompt on cloud-hosted devices. By performing GUI trajectory scraping and a final trajectory verification by many annotators, the system captures high-quality interaction data. Moreover, by %iteratively updating our UI-Venus-1.5 as the executor, 
% % iteratively feeding the valid trajectories to the MLLM as the examples for task prompt generation, the success rate of total trace generation pipeline raises from 17.9\% to over 70\%. In total, this pipeline produced more than 30,000 verified trajectories.
% To further improve robustness in real-world environments, we augment the Mid-Training corpus with interaction trajectories collected from real-device execution. Compared with static open-source datasets, real-device interaction data better captures execution failures, GUI dynamics, and environment-dependent behaviors that GUI agents must handle in practice.
% We therefore build a data generation loop on top of our DaaS system (Section~\ref{sec:daas}). As illustrated in Figure~\ref{fig:daas_feedback}, an open-source MLLM first generates candidate task prompts from seed instructions. After semantic verification based on embedding similarity, valid and non-duplicate prompts are stored in a task bank and executed by GUI agents on cloud-hosted devices. The system then performs GUI trajectory scraping followed by multi-annotator verification to collect high-quality interaction trajectories.
% A key feature of this pipeline is its iterative generation loop. Verified trajectories are fed back to the MLLM as in-context examples for subsequent task generation, enabling progressively more executable and realistic task prompts. As a result, the success rate of the trajectory generation pipeline improves from 17.9\% to over 70\% after several iterations.
% In total, this real-device generation loop produces more than 30,000 verified interaction trajectories.

\subsection{Data Verify}\label{sec:verify}

==> tables/ablation.tex <==

\begin{table}[ht]
    \centering
    % \footnotesize
    % \setlength{\tabcolsep}{0pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l *{9}{c}}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Mid-Training}}  & \multicolumn{2}{c}{\textbf{Offline-RL}} & \multicolumn{2}{c}{\textbf{Online-RL}} & \multicolumn{2}{c}{\textbf{Model Merge}} \\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9} 
    & \textbf{SS-Pro} & \textbf{AW} & \textbf{SS-Pro} & \textbf{AW} & \textbf{SS-Pro} & \textbf{AW}     & \textbf{SS-Pro} & \textbf{AW}     \\ 
    \midrule
    \rowcolor{gray!17}
    \multicolumn{9}{l}{\textit{UI-Venus-1.5}} \\
    \textbf{2B}    & 52.3 &39.0 & \textbf{59.0}(\textcolor{red}{+6.7$\uparrow$}) &45.3(\textcolor{red}{+6.3$\uparrow$})&- & \textbf{59.8}(\textcolor{red}{+14.5$\uparrow$}) & 57.7(\textcolor{green}{-1.3$\downarrow$})&    55.6 (\textcolor{green}{-4.2$\downarrow$})                       \\ 
    \textbf{8B}    & 63.1  &57.0 & \textbf{70.0}(\textcolor{red}{+6.9$\uparrow$}) & 63.5(\textcolor{red}{+6.5$\uparrow$})&- & 72.7(\textcolor{red}{+9.2$\uparrow$}) & 68.4(\textcolor{green}{-1.6$\downarrow$})&                           \textbf{73.7}(\textcolor{red}{+1.0$\uparrow$}) \\ 
    \textbf{30B-A3B}    & 65.2 &67.1 & \textbf{71.0}(\textcolor{red}{+5.8$\uparrow$})&68.0(\textcolor{red}{+0.9$\uparrow$}) &- & 75.5(\textcolor{red}{+7.5$\uparrow$})  &69.6(\textcolor{green}{-1.4$\downarrow$})&                           \textbf{77.6}(\textcolor{red}{+2.1$\uparrow$}) \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation studies of UI-Venus-1.5} on ScreenSpot-Pro (denote as ``SS-Pro'') and AndroidWorld (denote as ``AW'').}
    \label{tab:ablation}
\end{table}



==> tables/androidlab_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Gemini-1.5-Pro~\citep{team2024gemini}                      &  -    & 16.7                           \\ 
    GLM4-9B-ft~\citep{glm2024chatglm}                      &  9B    &  21.0                        \\ 
    LLaMA3.1-ft~\citep{grattafiori2024llama}                      &  8B    & 23.9                         \\ 
    GPT-4o~\citep{hurst2024gpt}       &   -        & 31.2  \\
    Qwen3-VL-2B\textsuperscript{*}~\citep{Qwen3-VL}   &  2B    & 33.3                           \\ 
    Qwen3-VL-8B\textsuperscript{*}~\citep{Qwen3-VL}  &  8B    &       43.5                  \\ 
    Qwen3-VL-30B-A3B\textsuperscript{*}~\citep{Qwen3-VL}  &  30B &      42.0                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
    AutoGLM~\citep{liu2024autoglm}       & -        & 36.2  \\
    V-Droid~\citep{dai2025advancing}  & 8B   & 38.3           \\
    UI-Genie~\citep{xiao2025ui} & 72B & 41.2  \\
    MobileUse~\citep{li2025mobileuse}  & 72B   & 44.2    \\
    UI-Venus-1.0-7B~\citep{gu2025ui} & 7B   &   41.3  \\
    UI-Venus-1.0-72B~\citep{gu2025ui} & 72B   &  49.3   \\
    AutoGLM-Mobile~\citep{liu2024autoglm}  & 9B   & 46.8    \\
    AutoGLM-Phone-9B-Multilingual~\citep{liu2024autoglm}  & 9B   & 47.7    \\
    Step-GUI-4B\textsuperscript{*}~\citep{yan2025step}  &  4B     &  47.8              \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &             \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &                \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{AndroidLab} for end-to-end models. \textsuperscript{*} indicates that the results were evaluated by us. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:AndroidLab}
\end{table}


==> tables/aw_and_al.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    % 减小列间距，确保两个表格能在一行放下
    \setlength{\tabcolsep}{1.5pt} 
    
    % --- 第一个表格 (左侧) ---
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \begin{tabular}{lcc}
        \toprule
        \textbf{Models} &\textbf{Params.}   & \textbf{Success Rate}                  \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{General VLMs}} \\
        Qwen3-VL-2B~\citep{Qwen3-VL}                       &  2B    & 36.4                                   \\ 
        Qwen3-VL-8B ~\citep{Qwen3-VL}                       &  8B    & 47.6                                  \\ 
        Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                       &  30B    &  54.3                        \\ 
        % GLM-4.6V-Flash~\citep{vteam2025glm45vglm41vthinkingversatilemultimodal}       &   9B        & 42.7  \\
        GLM-4.6V~\citep{vteam2025glm45vglm41vthinkingversatilemultimodal}       &   106B        & 57.0  \\
        Gemini-2.5-Pro~\citep{comanici2025gemini}  & -   &                     69.7       \\ 
        Seed1.8~\citep{seed1.8}  & -   &                     70.7       \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
        % ScaleCUA-3B~\citep{}                       &  3B         & 23.7                                   \\ 
        UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                       &  7B      & 30.0                       \\ 
        GUI-Owl-7B ~\citep{ye2025mobile}                       &  7B      &  66.4                      \\ 
        UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui}                &   72B     & 46.6  \\
        UI-Venus-1.0-7B~\citep{gu2025ui}                  &  7B & 49.1               \\ 
        UI-Venus-1.0-72B~\citep{gu2025ui}                 &  72B      & 65.9                \\
        %OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} &  30B      &                  \\
        Step-GUI-4B~\citep{yan2025step}  &  4B      & 63.9                \\ 
        Step-GUI-8B~\citep{yan2025step}                       &  8B      &                 67.7       \\ 
        Holo2-8B~\citep{hai2025holo2modelfamily}                       &  8B      & 60.4                       \\ 
        Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                       &  30B      &  71.6                       \\ 
        MAI-UI-2B~\citep{zhou2025mai}                       &  2B      &    49.1                   \\ 
        MAI-UI-8B~\citep{zhou2025mai}                       &  8B      &  70.7                   \\ 
        MAI-UI-32B~\citep{zhou2025mai}                       &  32B      &  73.3                   \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{Ours}} \\
        \textbf{UI-Venus-1.5-2B}               &  2B &      55.6        \\ 
        \textbf{UI-Venus-1.5-8B}               &  8B &      73.7        \\ 
        \textbf{UI-Venus-1.5-30B-A3B}               &  30B      &     \textbf{77.6} \\
        \bottomrule
        \end{tabular}
        \vspace{0.4em}
        \caption{Performance comparison on \textbf{AndroidWorld} for end-to-end models. 
        %Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.
        }
        \label{tab:Androidworld}
    \end{minipage}
    \hfill % 这里是关键，把两个minipage推向两边
    % --- 第二个表格 (右侧) ---
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \begin{tabular}{lcc}
        \toprule
        \textbf{Models} &\textbf{Params.}   & \textbf{Success Rate}                  \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{General VLMs}} \\
        Gemini-1.5-Pro~\citep{team2024gemini}                       &  -    & 16.7                                   \\ 
        GLM4-9B-ft~\citep{glm2024chatglm}                       &  9B    &  21.0                         \\ 
        LLaMA3.1-ft~\citep{grattafiori2024llama}                       &  8B    & 23.9                                  \\ 
        GPT-4o~\citep{hurst2024gpt}       &   -        & 31.2  \\
        Qwen3-VL-2B\textsuperscript{*}~\citep{Qwen3-VL}    &  2B    & 33.3                                   \\ 
        Qwen3-VL-8B\textsuperscript{*}~\citep{Qwen3-VL}   &  8B    &       43.5                  \\ 
        Qwen3-VL-30B-A3B\textsuperscript{*}~\citep{Qwen3-VL}   &  30B &       42.0                  \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{GUI-specific Models\&Frameworks}} \\
        %AutoGLM~\citep{liu2024autoglm}       & -        & 36.2  \\
        V-Droid~\citep{dai2025advancing}   & 8B   & 38.3            \\
        UI-Genie~\citep{xiao2025ui} & 72B & 41.2  \\
        MobileUse~\citep{li2025mobileuse}  & 72B   & 44.2     \\
        UI-Venus-1.0-7B~\citep{gu2025ui} & 7B   &   41.3  \\
        UI-Venus-1.0-72B~\citep{gu2025ui} & 72B   &  49.3    \\
        AutoGLM-Mobile~\citep{liu2024autoglm}  & 9B   & 46.8     \\
        AutoGLM-Multilingual~\citep{liu2024autoglm}  & 9B   & 47.7     \\
        Step-GUI-4B\textsuperscript{*}~\citep{yan2025step}   &  4B      &  47.8               \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{Ours}} \\
        \textbf{UI-Venus-1.5-2B}               &  2B &  36.2/44.2$^{\dagger}$            \\ 
        \textbf{UI-Venus-1.5-8B}               &  8B &  \textbf{55.1}/68.1$^{\dagger}$            \\ 
        \textbf{UI-Venus-1.5-30B-A3B}          &  30B & 52.9/68.1$^{\dagger}$             \\ 
        \bottomrule
        \end{tabular}
        \vspace{0.4em}
        \caption{Performance comparison on \textbf{AndroidLab}. Note that \textsuperscript{*} indicates that the results are evaluated by us; \textsuperscript{$\dagger$} denotes results that have been manually verified by humans.
        }
        \label{tab:AndroidLab}
    \end{minipage}
\end{table}

==> tables/cagui_exp.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lccc}
    \toprule
    \textbf{Models} & \textbf{Fun2Point} & \textbf{Text2Point}    & \textbf{Avg}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{4}{l}{\textit{Closed-source Models}} \\
    GPT-4o~\citep{openai2024gpt4o}                           & 22.1          & 19.9                 &            21.0             \\ 
    GPT-4o w grounding~\citep{openai2024gpt4o}                           & 44.3          & 44.0                 &   44.2    \\        
    \midrule
    \rowcolor{gray!15}
    \multicolumn{4}{l}{\textit{Open-source Models}} \\
    Intern2.5-VL-8B~\citep{chen2024expanding}                      & 17.2          & 24.2                          &     20.7        \\ 
    Intern2.5-VL-26B~\citep{chen2024expanding}                      & 14.8          & 16.6                        &        15.7      \\ 
    Qwen2.5-VL-7B~\citep{bai2025qwen25vltechnicalreport}                      & 59.8          & 59.3                &   59.6                     \\ 
    OS-Genesis-7B~\citep{osgenesis}                        & 8.3          & 5.8                 &   7.1    \\
    OS-Atlas-7B~\citep{wu2024osatlasfoundationactionmodel}                 & 53.6          & 60.7                 &   57.2           \\
    Aguvis-7B~\citep{xu2024aguvis}                        & 60.8          & 76.5                 &                68.7         \\
    UI-TARS-7B~\citep{qin2025uitarspioneeringautomatedgui}                        & 56.8          & 66.7                 &         61.8                 \\
    AgentCPM-GUI~\citep{agentcpm}                        & 79.1&76.5                &        77.8                \\
    \midrule
    \rowcolor{gray!15}
    \multicolumn{4}{l}{\textit{Ours}} \\
    UI-Venus-Ground-7B                        & { \ul 83.3} &  { \ul 83.2} & { \ul 83.3}         \\ 
    UI-Venus-Ground-72B                        & \textbf{84.1} & \textbf{85.9}        & \textbf{85.0}               \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{CA-GUI} grounding dataset. Our UI-Venus-72B achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:AgentCPM-GUI}
\end{table}


==> tables/gd_data.tex <==
% \begin{table*}[h]
% \centering
% \begin{tabular}{c|ccccc|c}
% \toprule
%                       & \textbf{widge\_captioning} & \textbf{UI\_refexp} & \textbf{Seeclick} & \textbf{ShowUI} & \textbf{Omniact} & \textbf{Total} \\ \hline
% \textbf{\#Samples} & 32742                      & 13084               & 38146             & 19435           & 3721             & 107128         \\ \bottomrule
% \end{tabular}
% \label{groundingdata}
% \caption{Basic statistics for grounding training data from different datasets.}
% \end{table*}



% \begin{table}[h]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{8pt}
% \begin{tabular}{l c}
% \toprule
% \textbf{Dataset} & \textbf{\# Samples} \\
% \midrule
% Widget Captioning & 32,742 \\
% UI RefExp & 13,084 \\
% SeeClick & 38,146 \\
% ShowUI & 19,435 \\
% OmniAct & 3,721 \\
% \midrule
% \textbf{Total} & \textbf{107,128} \\
% \bottomrule
% \end{tabular}
% \vspace{0.3em}
% \caption{Training data composition for GUI grounding tasks across different datasets.}
% \label{tab:grounding_data}
% \end{table} 

% \begin{table*}[h]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{c*{6}{c}} 
% \toprule
% \textbf{} & \textbf{Widget Captioning} & \textbf{UI RefExp} & \textbf{SeeClick} & \textbf{ShowUI} & \textbf{OmniAct} & \textbf{Total} \\
% \midrule
% \textbf{\# Samples} & 32,742 & 13,084 & 38,146 & 19,435 & 3,721 & \textbf{107,128} \\
% \bottomrule
% \end{tabular}
% \vspace{0.4em}
% \caption{Training data composition for GUI grounding tasks. Our training dataset comprises 107K samples from five complementary sources.}
% \label{tab:grounding_data}
% \end{table*}



\begin{table*}[h]\small
\centering
% \footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c|ccccc|c}
\toprule
\textbf{} & \textbf{Widget Captioning} & \textbf{UI RefExp} & \textbf{SeeClick-Web} & \textbf{ShowUI} & \textbf{OmniAct} & \textbf{Sampled training set} \\
\midrule
\textbf{\# Samples} & 34k & 17k & 325k & 110k & 141k  & \textbf{107k} \\
\bottomrule
\end{tabular}
\vspace{0.4em}
\caption{GUI grounding data composition. Our training dataset comprises 107k samples from five complementary sources.}
\label{tab:grounding_data}
\end{table*}

==> tables/mmbench.tex <==
\begin{table*}[t]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l *{13}{c}}
		\toprule
		\multirow{2}{*}{\textbf{Model}} &
		\multicolumn{2}{c}{\textbf{Windows}} &
		\multicolumn{2}{c}{\textbf{MacOS}} &
		\multicolumn{2}{c}{\textbf{Linux}} &
		\multicolumn{2}{c}{\textbf{iOS}} &
		\multicolumn{2}{c}{\textbf{Android}} &
		\multicolumn{2}{c}{\textbf{Web}} &
		\multirow{2}{*}{\textbf{Avg.}} \\
		\cmidrule(lr){2-3}
		\cmidrule(lr){4-5}
		\cmidrule(lr){6-7}
		\cmidrule(lr){8-9}
		\cmidrule(lr){10-11}
		\cmidrule(lr){12-13}
		& Bas. & Adv. & Bas. & Adv. & Bas. & Adv. & Bas. & Adv. & Bas. & Adv. & Bas. & Adv. & \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{14}{l}{\textit{General VLMs}} \\
		% Seed1.8~\citep{seed1.8}                         & - & - & - & - & - & - & - & - & - & - & - & - & 64.3 \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}              & 82.3 & 41.2 & 79.1 & 45.4 & 67.5 & 44.4 & 92.0 & 68.2 & 91.6 & 69.6 & 85.8 & 52.9 & 69.5 \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 82.05 & 67.91 & 57.62 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}             & 88.6 & 62.5 & 86.1 & 66.8 & 72.8 & 57.1 & 95.9 & 83.9 & 95.8 & 84.8 & 94.8 & 72.7 & 81.4 \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}          & 87.8 & 69.9 & 85.2 & 68.8 & 78.0 & 60.7 & \underline{96.5} & 84.5 & 96.3 & 88.5 & \underline{96.5} & 78.6 & 83.7 \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{14}{l}{\textit{GUI-specific Models}} \\
		% OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - & - & - & - & - & - & - & 50.0 \\
		% OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - & - & - & - & - & - & - & 55.3 \\
		% OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - & - & - & - & - & - & - & 60.8 \\
		% GTA1-7B~\citep{yang2025gta1guitesttimescaling}                          & - & - & - & - & - & - & - & - & - & - & - & - & 50.1 \\
		% GTA1-32B~\citep{yang2025gta1guitesttimescaling}                         & - & - & - & - & - & - & - & - & - & - & - & - & {63.6} \\
		GUI-Owl-7B~\citep{ye2025mobile}                       & 86.4 & 61.8 & 81.7 & 64.5 & 74.4 & 61.7& 94.9 & 83.0 & 95.8 & 83.7 & 93.2 & 72.7& 80.5 \\
		GUI-Owl-32B~\citep{ye2025mobile}                      & 85.6 & 65.1 & 84.9& 67.1 & 77.0 & 63.3& 95.2 & 85.5 & 96.1 & 87.0 & 95.5 & 80.8& 83.0 \\
		% UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 35.7 \\
		% UI-Venus-1.0-7B~\citep{gu2025ui}                  & - & - & - & - & - & - & - & - & - & - & - & - & 50.8 \\
		% UI-Venus-1.0-72B~\citep{gu2025ui}                 & - & - & - & - & - & - & - & - & - & - & - & - & {61.9} \\
		% OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} & - & - & - & - & - & - & - & - & - & - & - & - & 55.5\\
		Holo2-8B~\citep{hai2025holo2modelfamily}                         & 90.8 & 70.2 & 87.5 & 71.4 & 78.5 & 60.2 & 96.2 & 88.2 & 96.3 & 87.9 & 95.5 & 77.9 & 84.5 \\
		Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                    & 91.9 & 72.8 & 88.1 & 74.9 & 84.3 & 67.3 & \underline{96.5} & 89.7 & 96.3 & 90.1 & \underline{96.5} & 82.5 & 86.8 \\
		Step-GUI-4B~\citep{yan2025step}                      & - & - & - & - & - & - & - & - & - & - & - & - & 84.0 \\
		Step-GUI-8B~\citep{yan2025step}                      & - & - & - & - & - & - & - & - & - & - & - & - & 85.6 \\
		MAI-UI-2B~\citep{zhou2025mai}                        &84.9 &64.0 &89.3 &72.5 &75.4 &60.2 &95.2 &85.2 &96.3 &84.2 &92.9 &76.0 & 82.6 \\
		MAI-UI-8B~\citep{zhou2025mai}                        & 92.3 & 74.3 & \underline{90.7} & \underline{86.4} & 81.2 & 67.3 & \textbf{97.1} & 90.0 & \underline{97.5} & 92.7 & 95.8 & 86.0 & \underline{88.8}\\
		MAI-UI-32B~\citep{zhou2025mai}                       & \textbf{93.0} & \textbf{78.7} & \textbf{92.8} & \textbf{87.6} & \textbf{86.9} & \textbf{77.6} & \textbf{97.1} & \underline{92.4} & \textbf{98.0} & \underline{93.2} & 96.1 & \textbf{92.5} & \textbf{91.3}\\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{14}{l}{\textit{Ours}} \\
		UI-Venus-1.5-2B                       & 88.2 & 61.8 & 82.3 & 65.6 & 77.0 & 60.7 & 92.7 & 80.3 & 93.3 & 83.9 & 94.8 & 72.1 & 80.3 \\
		UI-Venus-1.5-8B                       & \underline{92.6} & 74.6 & 86.1 & 82.1 & 84.3 & 67.3 & \textbf{97.1} & 89.4 & 96.9 & 92.4 & \textbf{96.8} & 86.0 & 88.1 \\
		UI-Venus-1.5-30B-A3B                      & 91.5 & \underline{76.5} & 88.1 & 76.6 & \underline{85.9} & \underline{69.9} & \underline{96.5} & \textbf{93.0} & 97.2 & \textbf{93.8} & \underline{96.5} & \underline{87.7} & 88.6 \\
		\bottomrule
	\end{tabular*}
	\caption{Performance comparison on \textbf{MMbench-GUI-L2}. For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.}
	\label{tab:mmbench_gui_l2}
\end{table*}


==> tables/navi_data.tex <==
% \begin{table*}[h]
% \centering
% \begin{tabular}{c|ccccccc|cc}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}}           & \multicolumn{7}{c|}{\textbf{Multiple Steps}}                                                                                                                                                                         & \multicolumn{2}{c}{\textbf{Single Step}}          \\ 
%  & \multicolumn{1}{c}{\textbf{GUI-O}} & \multicolumn{1}{c}{\textbf{AITZ}} & \multicolumn{1}{c}{\textbf{AC}} & \multicolumn{1}{c}{\textbf{Aitw}}  & \multicolumn{1}{c}{\textbf{Amex}}  & \multicolumn{1}{c}{\textbf{CN-Navi*}} & \textbf{Total}  & \multicolumn{1}{c}{\textbf{GD*}} & \textbf{VQA*} \\ \hline
% \textbf{\#Samples}     & \multicolumn{1}{c}{114130}      & \multicolumn{1}{c}{13426}  & \multicolumn{1}{c}{84189}           & \multicolumn{1}{c}{35018} & \multicolumn{1}{c}{40153} & \multicolumn{1}{c|}{11037}       & 222183 & \multicolumn{1}{c}{107128}     & 41936   \\ \
% \textbf{\#Traces}    & \multicolumn{1}{c}{7406}        & \multicolumn{1}{c}{2099}   & \multicolumn{1}{c}{13353}           & \multicolumn{1}{c}{4324}  & \multicolumn{1}{c}{5674}  & \multicolumn{1}{c|}{1245}        & 34101  & \multicolumn{1}{c}{107128}     & 41936   \\ 
% \textbf{Length} & \multicolumn{1}{c}{15.4}        & \multicolumn{1}{c}{6.4}    & \multicolumn{1}{c}{6.3}             & \multicolumn{1}{c}{8.1}   & \multicolumn{1}{c}{9.3}   & \multicolumn{1}{c|}{8.9}         & 6.5    & \multicolumn{1}{c}{1.0}        & 1.0     \\ \bottomrule
% \end{tabular}

% \caption{Basic statistics for navigation training data, comparing both our annotated dataset and different open-source data. Note that ``AC'' means Android Control dataset while the ``GUI-O'' represents GUI-Odyssey. We report the number of traces and their average lengths. The dataset marked with * means our collected.}
% \label{tab:navidata}
% \end{table*}

\begin{table*}[h]\small
\centering
% \footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c|cccccc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Dataset}}           & \multicolumn{6}{c|}{\textbf{Multiple Steps}}                                                                                                                                                                         & \multicolumn{2}{c|}{\textbf{Single Step}}  & \multirow{2}{*}{\textbf{Sampled training set}}       \\ 
 & \multicolumn{1}{c}{{GUI-O}} & \multicolumn{1}{c}{{AITZ}} & \multicolumn{1}{c}{{AC}} & \multicolumn{1}{c}{{Aitw}}  & \multicolumn{1}{c}{{Amex}}  & \multicolumn{1}{c|}{{Navi*}}  & \multicolumn{1}{c}{{GD*}} & \multicolumn{1}{c|}{{VQA*}} &  \\ \hline
\textbf{\#Samples}     & \multicolumn{1}{c}{114k}      & \multicolumn{1}{c}{14k}  & \multicolumn{1}{c}{84k}           & \multicolumn{1}{c}{371k} & \multicolumn{1}{c}{39k} & \multicolumn{1}{c|}{20k}        & \multicolumn{1}{c}{107k}     & 42k & \textbf{350k}  \\ \
\textbf{\#Traces}    & \multicolumn{1}{c}{7k}        & \multicolumn{1}{c}{2k}   & \multicolumn{1}{c}{13k}           & \multicolumn{1}{c}{5k}  & \multicolumn{1}{c}{3k}  & \multicolumn{1}{c|}{*}          & \multicolumn{1}{c}{-}     & -  & * \\ \bottomrule
%\textbf{Length} & \multicolumn{1}{c}{15.4}        & \multicolumn{1}{c}{6.4}    & \multicolumn{1}{c}{6.3}             & \multicolumn{1}{c}{8.1}   & \multicolumn{1}{c}{9.3}   & \multicolumn{1}{c|}{8.9}         & 6.5    & \multicolumn{1}{c}{1.0}        & 1.0     \\ \bottomrule
\end{tabular}
\caption{Basic statistics for our collected navigation training data. Note that ``AC'' means Android Control dataset while the ``GUI-O'' represents GUI-Odyssey. The datasets marked with * means are collected by ourselves. Among these data, we select 350k high-quality samples as our training set.}
\label{tab:navidata}
\end{table*}


% multiple steps
% GUI-O：41300
% AITZ：10363 + 1647
% AITW：16410
% AC：42569
% Amex：34089
% Navi: 17685

% sinple steps
% GD：40000
% VQA：39006
% LOW：100000

==> tables/navi_online_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Qwen3-VL-2B~\citep{Qwen3-VL}                      &  2B    & 36.4                            \\ 
    Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    & 47.6                         \\ 
    Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &  54.3                       \\ 
    GLM-4.6V-Flash~\citep{vteam2025glm45vglm41vthinkingversatilemultimodal}       &   9B        & 42.7  \\
    GLM-4.6V~\citep{vteam2025glm45vglm41vthinkingversatilemultimodal}       &   106B        & 57.0  \\
    Gemini-2.5-Pro~\citep{comanici2025gemini}  & -   &                    69.7      \\ 
    Seed1.8~\citep{seed1.8}  & -   &                    70.7      \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
    ScaleCUA-3B~\citep{}                      &  3B         & 23.7                           \\ 
    UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                      &  7B     & 30.0                     \\ 
    GUI-Owl-7B ~\citep{ye2025mobile}                      &  7B     &  66.4                    \\ 
    UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui}               &   72B    & 46.6  \\
    UI-Venus-1.0-7B~\citep{gu2025ui}                 &  7B & 49.1             \\ 
    UI-Venus-1.0-72B~\citep{gu2025ui}                &  72B     & 65.9               \\
    %OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} &  30B     &                \\
    Step-GUI-4B~\citep{yan2025step}  &  4B     & 63.9               \\ 
    Step-GUI-8B~\citep{yan2025step}                      &  8B     &                67.7      \\ 
    Holo2-8B~\citep{hai2025holo2modelfamily}                      &  8B     & 60.4                     \\ 
    Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                      &  30B     &  71.6                     \\ 
    MAI-UI-2B~\citep{zhou2025mai}                      &  2B     &    49.1                  \\ 
    MAI-UI-8B~\citep{zhou2025mai}                      &  8B     &  70.7                    \\ 
    MAI-UI-32B~\citep{zhou2025mai}                      &  32B     &  73.3                    \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &             \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &                \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{AndroidWorld} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:Androidworld}
\end{table}


==> tables/odysseys.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model} & \textbf{Params.} &
\multicolumn{2}{c}{\textbf{Rubrics (\%) ($\uparrow$)}} \\
\cmidrule(lr){3-4}
& & \textbf{Averaged} & \textbf{Perfect} \\
\midrule
\rowcolor{gray!15}
\multicolumn{4}{@{}l}{\textit{General VLMs}} \\
Opus 4.6~\citep{anthropic2026opus46} & - & 68.9 & 44.5 \\
GPT-5.4~\cite{singh2025openai} & - & 55.4 & 33.5 \\
Sonnet 4.6~\citep{anthropic2026sonnet46} & - & 49.8 & 31.0 \\
GPT-5.4-mini~\cite{singh2025openai} & - & 38.4 & 10.5 \\
Seed-2.0~\citep{seed2} & - & 60.2 & 30.1 \\
Qwen-3.5-4B~\citep{qwen3.5} & - & 42.9 & 10.7 \\
Qwen-3.5-9B~\citep{qwen3.5} & - & 42.6 & 13.5 \\
Qwen-3.6-27B~\citep{qwen3.5} & - & -- & -- \\
Qwen-3.5-35B-A3B~\citep{qwen3.5} & - & 28.5 & 6.5 \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{GUI-specific Models}} \\
UI-TARS-1.5-7B~\citep{ui-tars-15-seed} & 7B & 10.0 & 1.0 \\
UI-Venus-1.5-32B~\citep{ui-tars-15-seed} & 32B & -- & -- \\
GUI-Owl-1.5-8B-Thinking \cite{xu2026mobile} & 8B & \\
GUI-Owl-1.5-32B-Thinking \cite{xu2026mobile} & 32B & \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{Ours}} \\
UI-Venus-2.0-9B & 9B & & \\
UI-Venus-2.0-27B & 27B & & \\
\bottomrule
\end{tabular}
\vspace{0.3em}
\caption{Performance comparison on \textbf{Odysseys}. UI-Venus-2.0 achieves state-of-the-art performance across model scales.}
\label{tab:webvoyager}
\end{table}


==> tables/online_mind2web.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model} & \textbf{Params.} &
\multicolumn{2}{c}{\textbf{Rubrics (\%) ($\uparrow$)}} \\
\cmidrule(lr){3-4}
& & \textbf{Averaged} & \textbf{Perfect} \\
\midrule
\rowcolor{gray!15}
\multicolumn{4}{@{}l}{\textit{General VLMs}} \\
Qwen3.5-9B~\citep{qwen3.5} & 9B & -- \\
Qwen3.6-27B~\citep{qwen3.6-27b} & 27B & -- \\
Seed2.0~\citep{seed2} & -- & -- \\
Kimi-k2.6 \citep{} & -- & -- \\
Opus4.6 \citep{anthropic2026opus46} & -- & -- \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{GUI-specific Models}} \\
UI-TARS-1.5-7B~\citep{ui-tars-15-seed} & 7B & 10.0 & 1.0 \\
UI-Venus-1.5-32B~\citep{ui-tars-15-seed} & 32B & -- & -- \\
GUI-Owl-1.5-8B-Thinking \cite{xu2026mobile} & 8B & \\
GUI-Owl-1.5-32B-Thinking \cite{xu2026mobile} & 32B & \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{Ours}} \\
UI-Venus-2.0-9B & 9B & & \\
UI-Venus-2.0-27B & 27B & & \\
\bottomrule
\end{tabular}
\vspace{0.3em}
\caption{Performance comparison on \textbf{Odysseys}. UI-Venus-2.0 achieves state-of-the-art performance across model scales.}
\label{tab:webvoyager}
\end{table}


==> tables/online_venus_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    &    6.7                      \\ 
    Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &  8.7                        \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\ 
    GUI-Owl-7B ~\citep{ye2025mobile}                      &  7B     &    6.7                  \\ 
    % MA3(GUI-Owl-7B)~\citep{ye2025mobile}                      &  7B     &                      \\ 
    UI-Venus-1.0-7B~\citep{gu2025ui}                &  7B &   8.1          \\ 
    UI-Venus-1.0-72B~\citep{gu2025ui}              &  72B &     15.4        \\ 
    Step-GUI-4B~\citep{yan2025step}  &  4B     &        8.0      \\ 
    MAI-UI-2B~\citep{zhou2025mai}                      &  2B     &                      \\ 
    MAI-UI-8B~\citep{zhou2025mai}                      &  8B     &     12.7                 \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &     16.1        \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &     21.5           \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{VenusBench-Mobile} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:VenusBench-Mobile}
\end{table}


==> tables/osworld.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Model} & \textbf{Params.} & \textbf{Success Rate} \\
\midrule

\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{General VLMs}} \\
Qwen3.5-9B~\citep{qwen3.5} & 9B & 41.8 \\
Qwen3.5-27B~\citep{qwen3.5} & 27B & 56.2 \\
% Qwen3.5-397B-A17B~\citep{qwen3.5} & 397B-A17B & 62.2 \\
% Qwen3.5-122B-A10B~\citep{qwen3.5} & 122B-A10B & 58.0 \\
Qwen3.6-27B~\citep{qwen3.5} & 27B & - \\
Gemini 3.1 Pro & - & 64.0 \\
Seed 2.0 & - & 64.4 \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{GUI-specific Models}} \\
UI-TARS-1.5~\citep{ui-tars-15-seed} & & 84.8 \\
UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui} & 72B & -- \\
Fara~\citep{fara7b2025} & 7B & 73.5 \\
Fara-1.5~\citep{awadallah2026fara} & 9B & 86.6 \\
MolmoWeb-4B \cite{gupta2026molmoweb} & 4B & 75.2 \\
MolmoWeb-8B \cite{gupta2026molmoweb} & 9B & 78.2 \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{Ours}} \\
UI-Venus-2-4B
    & 4B  & -- \\
UI-Venus-2-9B
    & 9B  & -- \\
\bottomrule
\end{tabular}
\vspace{0.3em}
\caption{Performance comparison on \textbf{OSworld-verified}. UI-Venus-1.5 achieves state-of-the-art performance across model scales.}
\label{tab:webvoyager}
\end{table}


==> tables/osworld_g.tex <==
\begin{table*}[t]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l *{6}{c}}
		\toprule
		% \textbf{Models} & \textbf{Text Matching} & \textbf{Element Recognition} & \textbf{Layout Understanding}& \textbf{Fine-grained Manipulation}& \textbf{Refusal}   & \textbf{Avg}                  \\ 
		\textbf{Models} &
		\textbf{\begin{tabular}[c]{@{}c@{}}Text \\ Matching\end{tabular}} &
		\textbf{\begin{tabular}[c]{@{}c@{}}Element \\ Recognition\end{tabular}} &
		\textbf{\begin{tabular}[c]{@{}c@{}}Layout \\ Understanding\end{tabular}}&
		\textbf{\begin{tabular}[c]{@{}c@{}}Fine-grained \\ Manipulation\end{tabular}}&
		\textbf{Refusal} &
		\textbf{Avg} \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{7}{l}{\textit{General VLMs}} \\
		% Seed1.8~\citep{seed1.8}                         & - & 64.3 & - & - & - & - \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}              & 60.9 & 49.7 & 57.3 & 38.9 & 0.0 & 47.7 \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 82.05 & 67.91 & 57.62 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}             & 71.6 & 59.4 & 61.3 & 49.7 & 1.9 & 57.4 \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}          & 73.9 & 65.2 & 67.2 & 51.0 & 5.6 & 61.2 \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{7}{l}{\textit{GUI-specific Models}} \\
		OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & 55.3 \\
		OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & 59.6 \\
		% OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - \\
		GTA1-7B~\citep{yang2025gta1guitesttimescaling}                          & 42.1 & 65.7 & 62.7 & 56.1 & 0.0 & 55.1\\
		GTA1-32B~\citep{yang2025gta1guitesttimescaling}                         & 63.2 & \textbf{78.4} & 73.3 & \textbf{65.2} & 0.0 & 65.2\\
		GUI-Owl-7B~\citep{ye2025mobile}                       & 64.8 & 63.6 & 61.3 & 41.0 & - & 55.9 \\
		GUI-Owl-32B~\citep{ye2025mobile}                      & 67.0 & 64.5 & 67.2 & 45.6 & - & 58.0 \\
		UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                   & - & - & - & - & - & 52.8 \\
		UI-Venus-1.0-7B~\citep{gu2025ui}                 & 74.6 & 60.5 & 61.5 & 45.5 & - & 54.6 \\
		UI-Venus-1.0-72B~\citep{gu2025ui}                 & \textbf{82.1} & 71.2 & 70.7 & \underline{64.4} & - & 62.2 \\
		%OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} & -& 55.5& 96.3&-&-& -& - \\
		Holo2-8B*~\citep{hai2025holo2modelfamily}                         & 74.3 & 68.2 & 67.6 & 59.1 & 0.0 & 63.5 \\
		Holo2-30B-A3B*~\citep{hai2025holo2modelfamily}                    & 77.0 & 68.8 & 70.0 & 59.7 & 0.0 & 65.2 \\
		Step-GUI-4B*~\citep{yan2025step}                      & 70.1 & 65.8 & 67.6 & 53.0 & 0.0 & 60.5 \\
		% Step-GUI-8B~\citep{yan2025step}                      & - & - & - & - & - & - \\
		MAI-UI-2B~\citep{zhou2025mai}                        & 62.8 &56.7 &59.3 &40.3 &- & 52.0\\
		MAI-UI-8B~\citep{zhou2025mai}                        & 72.0 &63.3 &66.0 &51.0 &- & 60.1\\
		MAI-UI-32B~\citep{zhou2025mai}                       & 73.6 & 72.4 & \underline{73.9} & 57.7 & - & 67.6\\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{7}{l}{\textit{Ours}} \\
		UI-Venus-1.5-2B                       & 67.4 & 66.1 & 66.4 & 44.3 & 7.4 & 59.4 \\
		UI-Venus-1.5-8B                       & 79.7 & \underline{76.1} & 72.3 & 60.4 & \textbf{22.2} & \underline{69.7} \\
		UI-Venus-1.5-30B-A3B                      & \underline{80.1} & \underline{76.1} & \textbf{75.1} & 61.1 & \underline{9.3} & \textbf{70.6} \\
		\bottomrule
	\end{tabular*}
	\vspace{0.4em}
	\caption{Performance comparison on \textbf{OS-World-G}. For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.}
	% Our UI-Venus-72B achieves state-of-the-art performance with a significant lead on the Text Matching subtask.
	\label{tab:osworld_g}
\end{table*}


==> tables/osworld_g_r.tex <==
\begin{table*}[t]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l *{6}{c}}
		\toprule
		% \textbf{Models} & \textbf{Text Matching} & \textbf{Element Recognition} & \textbf{Layout Understanding}& \textbf{Fine-grained Manipulation}& \textbf{Refusal}   & \textbf{Avg}                  \\ 
		\textbf{Models} &
		\textbf{\begin{tabular}[c]{@{}c@{}}Text \\ Matching\end{tabular}} &
		\textbf{\begin{tabular}[c]{@{}c@{}}Element \\ Recognition\end{tabular}} &
		\textbf{\begin{tabular}[c]{@{}c@{}}Layout \\ Understanding\end{tabular}}&
		\textbf{\begin{tabular}[c]{@{}c@{}}Fine-grained \\ Manipulation\end{tabular}}&
		\textbf{Refusal} &
		\textbf{Avg} \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{7}{l}{\textit{General VLMs}} \\
		% Seed1.8~\citep{seed1.8}                         & - & 64.3 & - & - & - & - \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}              & 73.2 & 64.2 & 70.8 & 47.0 & 0.0 & 60.6 \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 82.05 & 67.91 & 57.62 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}             & 78.2 & 71.5 & 72.3 & 55.7 & 1.9 & 67.0 \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}          & 77.8 & 75.8 & 74.7 & 54.4 & 5.6 & 69.3 \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{7}{l}{\textit{GUI-specific Models}} \\
		% OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & 55.3 \\
		OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & 63.2 & 79.9 & \textbf{84.9} & 62.1 & 7.4 & 70.2 \\
		% OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - \\
		GTA1-7B~\citep{yang2025gta1guitesttimescaling}                          & 63.2 & \underline{82.1} & 74.2 & \textbf{70.5} & 0.0 & 67.7 \\
		GTA1-32B~\citep{yang2025gta1guitesttimescaling}                         & 63.2 & \textbf{83.6} & \underline{84.4} & \textbf{70.5} & 0.0 & 72.2 \\
		% GUI-Owl-7B~\citep{ye2025mobile}                       & 64.8 & 63.6 & 61.3 & 41.0 & - & 55.9 \\
		% GUI-Owl-32B~\citep{ye2025mobile}                      & 67.0 & 64.5 & 67.2 & 45.6 & - & 58.0 \\
		% UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                   & - & - & - & - & - & 52.8 \\
		UI-Venus-1.0-7B~\citep{gu2025ui}                 & 74.6 & 60.5 & 61.5 & 45.5 & - & 58.8 \\
		UI-Venus-1.0-72B~\citep{gu2025ui}                 & 82.1 & 71.2 & 70.7 & 64.4 & - & 70.4 \\
		%OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} & -& 55.5& 96.3&-&-& -& - \\
		Holo2-8B*~\citep{hai2025holo2modelfamily}                         & - & - & - & - & - & 70.1 \\
		Holo2-30B-A3B*~\citep{hai2025holo2modelfamily}                    & - & - & - & - & - & \underline{76.1} \\
		Step-GUI-4B*~\citep{yan2025step}                      & - & - & - & - & - & 66.9 \\
		% Step-GUI-8B~\citep{yan2025step}                      & - & - & - & - & - & - \\
		MAI-UI-2B~\citep{zhou2025mai}                        & 70.9 &69.1 &72.7 &47.7 &- & 63.5\\
		MAI-UI-8B~\citep{zhou2025mai}                        & 77.4 &73.0 &78.3 &55.7 &- & 68.6\\
		MAI-UI-32B~\citep{zhou2025mai}                       & 79.7 & 79.4 & 81.0 & 61.7 & - & 73.9\\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{7}{l}{\textit{Ours}} \\
		UI-Venus-1.5-2B                       & 75.1 & 70.0 & 73.5 & 52.3 & 7.4 & 65.6 \\
		UI-Venus-1.5-8B                       & \underline{82.4} & 81.5 & 80.2 & 59.7 & \textbf{22.2} & 74.1 \\
		UI-Venus-1.5-30B-A3B                      & \textbf{83.1} & \underline{82.1} & 83.4 & \underline{65.8} & \underline{9.3} & \textbf{76.4} \\
		\bottomrule
	\end{tabular*}
	\vspace{0.4em}
	\caption{Performance comparison on \textbf{OS-World-G-Refine}.
		% Our UI-Venus-72B achieves state-of-the-art performance with a significant lead on the Text Matching subtask.
		For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.
	}
	\label{tab:osworld_g}
\end{table*}


==> tables/real.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Model} & \textbf{Params.} & \textbf{Success Rate} \\
\midrule

\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{General VLMs}} \\
Qwen3.5-9B~\citep{qwen3.5} & 9B & 18.2 \\
Qwen3.6-27B~\citep{qwen3.6-27b} & 27B & -- \\
Qwen3.8-Max~\citep{qwen38} & - & 38.0 \\
Seed2.0~\citep{seed2} & -- & 70.2 \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{GUI-specific Models}} \\
GUI-Owl-1.5-8B-Instruct \cite{xu2026mobile} & 8B &  \\
GUI-Owl-1.5-8B-Thinking \cite{xu2026mobile} & 8B &  \\
GUI-Owl-1.5-32B-Thinking \cite{xu2026mobile} & 32B &  \\
Fara~\citep{fara7b2025} & 7B &  \\
MolmoWeb-4B \cite{gupta2026molmoweb} & 4B &  \\
MolmoWeb-8B \cite{gupta2026molmoweb} & 9B &  \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{Ours}} \\
UI-Venus-2-9B & 9B  & -- \\
UI-Venus-2-27B & 27B  & -- \\
\bottomrule
\end{tabular}
\vspace{0.3em}
\caption{Performance comparison on \textbf{OSworld-verified}. UI-Venus-1.5 achieves state-of-the-art performance across model scales.}
\label{tab:real}
\end{table}


==> tables/sspro_exp.tex <==
\begin{table*}[t]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l *{15}{c}}
		\toprule
		\multirow{3}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{CAD}} & \multicolumn{2}{c}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Creative}} & \multicolumn{2}{c}{\textbf{Scientific}} & \multicolumn{2}{c}{\textbf{Office}} & \multicolumn{2}{c}{\textbf{OS}} & \multicolumn{3}{c}{\textbf{Avg.}} \\
		\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-16}
		& Text & Icon & Text & Icon & Text & Icon & Text & Icon & Text & Icon & Text & Icon & Text & Icon & \textbf{Avg.} \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{16}{l}{\textit{General VLMs}} \\
		Seed1.8~\citep{seed1.8}                         & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 64.3 \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}              & 27.9 & 10.9 & 57.1 & 9.7 & 58.1 & 16.8 & 62.5 & 22.7 & 73.4 & 34.0 & 55.1 & 19.1 & 55.0 & 17.4 & {40.6} \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 82.05 & 67.91 & 57.62 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}             & 56.9 & 10.9 & 75.3 & 22.8 & 68.2 & 16.1 & 78.5 & 32.7 & 80.8 & 39.6 & 71.0 & 20.2 & 71.1 & 22.8 & 52.7 \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}          & 51.8 & 15.6 & 76.0 & 24.8 & 69.2 & 20.3 & 76.4 & 27.3 & 80.8 & 37.7 & 75.7 & 38.2 & 70.6 & 26.3 & 53.7 \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{16}{l}{\textit{GUI-specific Models}} \\
		OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 50.0 \\
		OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 55.3 \\
		OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 60.8 \\
		GTA1-7B~\citep{yang2025gta1guitesttimescaling}                          & 66.9   & 20.7   & 62.6   & 18.2   & 53.3   & 17.2   & 76.4 & 31.8   & 82.5   & 50.9   & 48.6  & 25.9   & 65.5   & 25.2   & 50.1 \\
		GTA1-32B~\citep{yang2025gta1guitesttimescaling}                         & \textbf{83.1} & {37.9} & {72.2} & {25.9} & {70.1} & 31.3 & {84.7} & {39.1} & {89.3} & {64.2} & {76.6} & {51.7} & {78.9} & {38.9} & {63.6} \\
		GUI-Owl-7B~\citep{ye2025mobile}                       & 64.5 & 21.9 & 76.6 & 31.0 & 59.6 & 27.3 & 79.1 & 37.3 & 77.4 & 39.6 & 59.8 & 33.7 & - & - & 54.9 \\
		GUI-Owl-32B~\citep{ye2025mobile}                      & 62.4 & 28.1 & {84.4} & 39.3 & 65.2 & 18.2 & 82.6 & 39.1 & 81.4 & 39.6 & 70.1 & 36.0 & - & - & 58.0\\
		% UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 35.7 \\
		UI-Venus-1.0-7B~\citep{gu2025ui}                  & {60.4} & 21.9  & {74.7} & 24.1  & 63.1  & {14.7} & {76.4} & 31.8  & 75.7  & 41.5  & {49.5} & 22.5  & {67.1} & 24.3  & 50.8 \\
		UI-Venus-1.0-72B~\citep{gu2025ui}                 & {66.5}  & {29.7}  & {84.4}  & {33.1} & {73.2} & {30.8}  & {84.7}  & {42.7} & {83.1} & {60.4}  & {75.7}  & {36.0} & {77.4}  & {36.8} & {61.9} \\
		% OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} &48.7 &23.4 &78.6 &31.7 &66.7 &22.4& 75.7 &34.56 &81.4 &47.2 &74.8 &43.8 & - & - &55.5\\
		Holo2-8B~\citep{hai2025holo2modelfamily}                         & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 58.9 \\
		Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                    & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 66.1 \\
		Step-GUI-4B~\citep{yan2025step}                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 60.0 \\
		Step-GUI-8B~\citep{yan2025step}                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 62.6 \\
		MAI-UI-2B~\citep{zhou2025mai}                        &61.4 &23.4 &76.6 &32.4 &69.2 &21.7 &81.2 &34.5 &85.9 &39.6 &68.2 &41.6 & - & -&57.4 \\
		MAI-UI-8B~\citep{zhou2025mai}                        &72.6 &35.9 &83.8 &52.4 &\underline{76.3} &33.6 &79.9 &37.3 & 88.7 &60.4 &76.6 &49.4 & - & -& 65.8\\
		MAI-UI-32B~\citep{zhou2025mai}                       &70.1 & \textbf{45.3} & \underline{86.4} &40.7 & \textbf{82.8} &\underline{37.8} & \textbf{91.7} &\underline{46.4} & \underline{90.4} &\textbf{71.7} & 78.5 &34.8 & - & -& 67.9\\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{16}{l}{\textit{Ours}} \\
		UI-Venus-1.5-2B                       & 54.3 & 32.8 & 70.1 & 43.4 & 63.6 & 28.7 & 76.4 & 38.2 & 81.9 & 47.2 & 73.8 & 51.7 & 69.1 & 39.4 & 57.7 \\
		UI-Venus-1.5-8B                       & \underline{75.1} & 31.2 & 85.7 & \underline{54.5} & 75.3 & 32.9 & \underline{86.1} & 44.5 & \textbf{92.7} & 66.0 & \underline{82.2} & \underline{52.8} & \textbf{82.4} & \underline{45.9} & \underline{68.4} \\
		UI-Venus-1.5-30B-A3B                      & 70.6 & \underline{40.6} & \textbf{87.7} & \textbf{57.9} & 75.8 & \textbf{41.3} & 84.0 & \textbf{47.3} & 89.8 & \underline{69.8} & \textbf{83.2} & \textbf{56.2} & \underline{81.2} & \textbf{51.0} & \textbf{69.6} \\
		\bottomrule
	\end{tabular*}
	\caption{Performance comparison on \textbf{ScreenSpot-Pro}. For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.}
	\label{tab:screenspot_pro}
\end{table*}


==> tables/ssv2_exp.tex <==
\begin{table}[ht]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l *{7}{c}}
		\toprule
		\multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Mobile}}  & \multicolumn{2}{c}{\textbf{Desktop}} & \multicolumn{2}{c}{\textbf{Web}}     & \multirow{2}{*}{\textbf{Avg}} \\
		\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
		& \textbf{Text} & \textbf{Icon/Widget} & \textbf{Text} & \textbf{Icon/Widget} & \textbf{Text} & \textbf{Icon/Widget} &                               \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{8}{l}{\textit{General VLMs}} \\
		% Seed1.8~\citep{seed1.8}                         & - & -  & - & - & - & - & - \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}              & 94.1 & 80.6 & 94.8 & 74.3 & 89.7 & 72.9 & 85.6 \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 82.05 & 67.91 & 57.62 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}             & \textbf{99.7} & 87.7 & 94.8 & 83.6 & 95.3 & 85.7 & 92.1 \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}          & 99.0 & 87.7 & 95.4 & 82.9 & 95.3 & 83.7 & 91.7 \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{8}{l}{\textit{GUI-specific Models}} \\
		OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & -  & - & - & - & - & 92.3 \\
		OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & -  & - & - & - & - & 93.4 \\
		OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & -  & - & - & - & - & 92.9 \\
		GTA1-7B~\citep{yang2025gta1guitesttimescaling}                          & 99.0 & 88.6 & 94.9 & 89.3 & 92.3 & 86.7 & 92.4  \\
		GTA1-32B~\citep{yang2025gta1guitesttimescaling}                         & \textbf{99.7} & 90.5 & \underline{99.0} & \textbf{94.3} & 95.7 & 90.1 & 95.2 \\
		GUI-Owl-7B~\citep{ye2025mobile}                       & 99.0 & 92.4 & 96.9 & 85.0 & 93.6 & 85.2 & 92.8 \\
		GUI-Owl-32B~\citep{ye2025mobile}                      & 98.6 & 90.0 & 97.9 & 87.8 & 94.4 & 86.7 & 93.2 \\
		% UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                   & - & -  & - & - & - & - & 91.6 \\
		UI-Venus-1.0-7B~\citep{gu2025ui}                  & 99.0  & 90.0         & 97.0  & 90.7 & 96.2 & 88.7       &      94.1               \\
		UI-Venus-1.0-72B~\citep{gu2025ui}                 & \textbf{99.7}  & \underline{93.8}        & 95.9  & 90.0 & 96.2 & 92.6         & 95.3      \\
		% OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} & \underline{99.3} & \underline{94.3} & \underline{99.0} & \textbf{96.4} & 97.4 & \underline{94.0} & \underline{96.3}\\
		Holo2-8B~\citep{hai2025holo2modelfamily}                         & - & -  & - & - & - & - & 93.2 \\
		Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                    & - & -  & - & - & - & - & 94.9 \\
		Step-GUI-4B~\citep{yan2025step}                      & - & -  & - & - & - & - & 93.6 \\
		Step-GUI-8B~\citep{yan2025step}                      & - & -  & - & - & - & - & 95.1 \\
		MAI-UI-2B~\citep{zhou2025mai}                        & \underline{99.3} &87.2 &97.4 &88.6 &94.0 &84.7 &92.5\\
		MAI-UI-8B~\citep{zhou2025mai}                        &\underline{99.3} &89.1 &\underline{99.0} &92.1 &\underline{97.9} &91.1 &95.2\\
		MAI-UI-32B~\citep{zhou2025mai}                       &99.0 &92.9 &\textbf{99.5} &\underline{93.6} &97.4 &\textbf{94.6} &\textbf{96.5}\\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{8}{l}{\textit{Ours}} \\
		UI-Venus-1.5-2B                       & 98.6 & 91.0 & 93.3 & 92.9 & 93.2 & 85.7 & 92.8 \\
		UI-Venus-1.5-8B                       & \underline{99.3} & 92.9 & 96.4 & 92.9 & \textbf{98.3} & \underline{93.1} & 95.9 \\
		UI-Venus-1.5-30B-A3B                      & \underline{99.3} & \textbf{94.8} & 95.9 & \textbf{94.3} & \underline{97.9} & \underline{93.1} & \underline{96.2} \\
		\bottomrule
	\end{tabular*}
	\vspace{0.4em}
	\caption{Performance comparison on \textbf{ScreenSpot-V2}. For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.}
	\label{tab:screenspot-v2}
\end{table}


==> tables/trainingdetails.tex <==
\begin{table}[ht]\small
\centering
% \footnotesize
\begin{tabular}{lccccc}
\toprule
    % save\_steps & 400 \\
\textbf{Hyperparameter} & \textbf{rollout} & \textbf{batch\_size} & \textbf{$\beta_{KL}$}  & \textbf{freeze\_vit} & \textbf{epoch}\\
\midrule
    \textbf{UI-Venus-Ground-7B}  & 8  & 128 & 4e-3 & False & 10  \\
    \textbf{UI-Venus-Ground-72B} & 10 & 128 & 4e-3 & False & 1  \\
    \textbf{UI-Venus-Navi-7B}    & 8  & 256 & 1e-3 & True  & 10  \\
   \textbf{UI-Venus-Navi-72B}    & 8  & 512 & 1e-3 & True  & 1 \\
\bottomrule
\end{tabular}
\vspace{0.4em}
\caption{Training hyperparameter settings used in the experiments of UI-Venus.}
\label{tab:hyper}
\end{table}

==> tables/uivision.tex <==
\begin{table}[ht]
	% \vspace{-1em}
	\centering
	\footnotesize
	%\setlength{\tabcolsep}{0pt}
	\begin{tabular}{lcccc}
		\toprule
		\textbf{Models}                                               & \textbf{Basic}   & \textbf{Functional} & \textbf{Spatial} & \textbf{Avg}     \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{5}{l}{\textit{General VLMs}}                                                                                                    \\
		% Seed1.8~\citep{seed1.8}                                       & -              & 64.3                & -                & -                \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}                                 & 16.4             & 19.1                & 4.6              & 13.1             \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}                                 & 27.8             & 29.6                & 9.4              & 21.9             \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}                            & 31.2             & 31.9                & 14.6             & 25.6             \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{5}{l}{\textit{GUI-specific Models}}                                                                                             \\
		OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}  & -                & -                   & -                & 29.7             \\
		OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse} & -                & -                   & -                & 33.3             \\
		OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse} & -                & -                   & -                & 37.3             \\
		% GTA1-7B~\citep{yang2025gta1guitesttimescaling}                & 46.4           & 50.1                & 92.4             & -                \\
		% GTA1-32B~\citep{yang2025gta1guitesttimescaling}               & 58.8           & 63.6                & 95.2             & -                \\
		% GUI-Owl-7B~\citep{ye2025mobile}                               & -              & 54.9                & 92.8             & -                \\
		% GUI-Owl-32B~\citep{ye2025mobile}                              & -              & 58.0                & 93.1             & -                \\
		% UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                        & 40.7           & 35.7                & 91.6             & 22.3             \\
		UI-Venus-1.0-7B~\citep{gu2025ui}                              & 36.1             & 32.8                & 11.9             & 26.5             \\
		UI-Venus-1.0-72B~\citep{gu2025ui}                             & 45.6             & 42.3                & 23.7             & 36.8             \\
		%OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} & -& 55.5& 96.3& - \\
		Holo2-8B*~\citep{hai2025holo2modelfamily}                     & 43.6             & 43.5                & 19.7             & 35.1             \\
		Holo2-30B-A3B*~\citep{hai2025holo2modelfamily}                & 51.0             & 50.1                & 23.2             & 40.9             \\
		Step-GUI-4B*~\citep{yan2025step}                              & 39.2             & 36.5                & 15.7             & 30.0             \\
		% Step-GUI-8B~\citep{yan2025step}                               & -              & 62.6                & 95.1             & -                \\
		MAI-UI-2B~\citep{zhou2025mai}                                 & 41.0             & 41.2                & 10.4             & 30.3             \\
		MAI-UI-8B~\citep{zhou2025mai}                                 & 51.7             & 49.6                & 22.5             & 40.7             \\
		MAI-UI-32B~\citep{zhou2025mai}                                & 59.1             & \underline{57.1}    & 26.9             & \underline{47.1} \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{5}{l}{\textit{Ours}}                                                                                                            \\
		% UI-Venus-1.5-2B-A100                       & 67.1 & 57.9 & 92.8 & 44.6 \\
		UI-Venus-1.5-2B                                               & \underline{63.5} & 51.5                & 21.6             & 44.8             \\
		% UI-Venus-1.5-8B-A100                       & \underline{72.0} & \underline{68.1} & 95.4 & 46.9 \\
		UI-Venus-1.5-8B                                               & 56.3             & 52.4                & \underline{32.0} & 46.5             \\
		UI-Venus-1.5-30B-A3B                                          & \textbf{69.0}    & \textbf{59.3}       & \textbf{37.4}    & \textbf{54.7}    \\
		\bottomrule

	\end{tabular}
	\vspace{0.4em}
	\caption{Performance comparison on \textbf{UI-Vision}. For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively.Asterisk (*) indicates results that may require verification with original sources.}
	\label{tab:ui-vison}
\end{table}


==> tables/venusbench_and_webvoyager.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    % 减小列间距，确保两个表格能在一行放下
    \setlength{\tabcolsep}{1.5pt} 
    
    % --- 第一个表格 (左侧) ---
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \footnotesize
        %\setlength{\tabcolsep}{0pt}
        \begin{tabular}{lcc}
        \toprule
        \textbf{Models} &\textbf{Params.}   & \textbf{Success Rate}                  \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{General VLMs}} \\
        Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    &    6.7                      \\ 
        Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &  8.7                        \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{GUI-specific Models}} \\ 
        GUI-Owl-7B ~\citep{ye2025mobile}                      &  7B     &    6.7                  \\ 
        % MA3(GUI-Owl-7B)~\citep{ye2025mobile}                      &  7B     &                      \\ 
        UI-Venus-1.0-7B~\citep{gu2025ui}                &  7B &   8.1          \\ 
        UI-Venus-1.0-72B~\citep{gu2025ui}              &  72B &     15.4        \\ 
        Step-GUI-4B~\citep{yan2025step}  &  4B     &        8.0      \\ 
        MAI-UI-2B~\citep{zhou2025mai}                      &  2B     &     6.7                 \\ 
        MAI-UI-8B~\citep{zhou2025mai}                      &  8B     &     12.7                 \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{Ours}} \\
        \textbf{UI-Venus-1.5-2B}              &  2B &      8.7       \\ 
        \textbf{UI-Venus-1.5-8B}              &  8B &     16.1        \\ 
        \textbf{UI-Venus-1.5-30B-A3B}              &  30B     &     \textbf{21.5}           \\ 
        \bottomrule
        \end{tabular}
        \vspace{0.4em}
        \caption{Performance comparison on \textbf{VenusBench-Mobile} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance on this challenging benchmark.}
        \label{tab:VenusBench-Mobile}
    \end{minipage}
    \hfill % 这里是关键，把两个minipage推向两边
    % --- 第二个表格 (右侧) ---
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \footnotesize
        %\setlength{\tabcolsep}{0pt}
        \begin{tabular}{lcc}
        \toprule
        \textbf{Models} &\textbf{Params.} & \textbf{Success Rate} \\ 
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{General VLMs}} \\
        Qwen3.5-9B~\citep{qwen3.5} & 9B & 46.9 \\
        Qwen3.6-27B~\citep{qwen3.6-27b} & 27B & 84.3 \\
        OpenAI Operator \citep{openai2025operator} & -- & 87.0 \\
        Seed2.0~\citep{seed2} & -- & 85.1 \\
        Glm-5v-turbo \citep{hong2026glm} & -- & 88.5 \\
        Opus4.6 \citep{anthropic2026opus46} & -- & 88.0 \\
        Kimi-k2.6 \citep{kimi-k2.6} & 1T & -- \\
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
        UI-TARS-1.5~\citep{ui-tars-15-seed} & -- & 84.8 \\
        Holo2-4B~\citep{hai2025holo2modelfamily} & 4B  & 80.2 \\
        Holo2-8B~\citep{hai2025holo2modelfamily} & 8B  & 80.2 \\
        Holo2-30B-A3B~\citep{hai2025holo2modelfamily} & 30B & 83.0 \\
        UI-Venus-1.5-2B \cite{team2026ui} & 2B & 56.4 \\
        UI-Venus-1.5-8B \cite{team2026ui} & 8B & 70.8 \\
        UI-Venus-1.5-30B-A3B \cite{team2026ui} & 30B & 76.0 \\
        GUI-Owl-1.5-8B-Instruct \cite{xu2026mobile} & 8B & 69.9 \\
        GUI-Owl-1.5-8B-Thinking \cite{xu2026mobile} & 8B & 78.1 \\
        GUI-Owl-1.5-32B-Thinking \cite{xu2026mobile} & 32B & 82.1 \\
        MolmoWeb-4B \cite{gupta2026molmoweb} & 4B & 75.2 \\
        MolmoWeb-8B \cite{gupta2026molmoweb} & 9B & 78.2 \\
        Fara~\citep{fara7b2025} & 7B & 73.5 \\
        Fara-1.5~\citep{awadallah2026fara} & 9B & 86.6 \\
        \midrule
        \rowcolor{gray!15}
        \multicolumn{3}{l}{\textit{Ours}} \\
        \textbf{UI-Venus-2-9B} & 9B & \\ 
        \textbf{UI-Venus-2-27B} & 27B & \\ 
        \bottomrule
        \end{tabular}
        \vspace{0.4em}
        \caption{Performance comparison on \textbf{Webvoyager} existing GUI Agents. Note that \textsuperscript{*} indicates that the results are evaluated by us.}
        \label{tab:webvoyager}
    \end{minipage}
\end{table}



==> tables/venusbench_gd.tex <==
\begin{table}[ht]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l *{9}{c}}
		\toprule
		\multirow{2}{*}{\textbf{Models}} &
		\multicolumn{4}{c}{\textbf{Basic Tasks}} &
		\multicolumn{4}{c}{\textbf{Advanced Tasks}} &
		\multirow{2}{*}{\textbf{Overall}} \\
		\cmidrule(lr){2-5} \cmidrule(lr){6-9}
		& \textbf{Element} & \textbf{Visual} & \textbf{Spatial} & \textbf{Avg} &
		\textbf{Reasoning} & \textbf{Functional} & \textbf{Refusal} & \textbf{Avg} & \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{10}{l}{\textit{General VLMs}} \\
		% Seed1.8~\citep{seed1.8}                         & - & -  & - & - & - & - & - \\
		Qwen3-VL-2B*~\citep{Qwen3-VL}              & 66.6 & 79.7 & 61.3 & 68.2 & 12.6 & 41.6 & 0.0 & 15.9 & 45.2 \\
		%Qwen3-VL-4B*~\citep{Qwen3-VL}                 & 51.28 & 55.53 & 91.67 & 82.05 & 67.91 & 57.62 & 21.66 \\
		Qwen3-VL-8B*~\citep{Qwen3-VL}             & 73.9 & 83.8 & 75.5 & 76.8 & 22.6 & 61.3 & 6.8 & 27.3 & 55.1 \\
		Qwen3-VL-30B-A3B*~\citep{Qwen3-VL}          & 68.0 & 84.3 & 69.2 & 72.3 & 19.9 & 58.6 & 11.3 & 27.0 & 52.4 \\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{10}{l}{\textit{GUI-specific Models}} \\
		OpenCUA-7B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & {62.23} & {84.39} & 67.44 & {69.15} & 21.32 & 49.14 & 0.00 & 21.43 & 48.20 \\
		OpenCUA-32B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & {65.49} & 78.55 & {68.80} & {69.64} & 29.09 & {51.00} & 0.00 & 25.08 & {50.08} \\
		% OpenCUA-72B~\citep{wang2025opencuaopenfoundationscomputeruse}                     & - & -  & - & - & - & - & - & - & 92.9 \\
		GTA1-7B~\citep{yang2025gta1guitesttimescaling}                          & 63.73 & 76.64 & 57.05 & 64.87 & 23.31 & 51.14 & 0.00 & 22.75 & 46.38 \\
		GTA1-32B~\citep{yang2025gta1guitesttimescaling}                         & 75.36 & 88.08 & 76.77 & 78.87 & 38.84 & 67.14 & 0.00 & 33.25 & 58.84 \\
		% GUI-Owl-7B~\citep{ye2025mobile}                       & - & - & - & - & - & - & - & - & 92.8 \\
		% GUI-Owl-32B~\citep{ye2025mobile}                      & - & - & - & - & - & - & - & - & 93.2 \\
		% UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                   & - & -  & - & - & - & - & 91.6 \\
		UI-Venus-1.0-7B~\citep{gu2025ui}                  & 64.30 & 78.78 & 67.15 & 68.66 & 24.39 & 53.85 & 0.00 & 23.90 & 49.01 \\
		UI-Venus-1.0-72B~\citep{gu2025ui}                 & {81.58} & {91.30} & {78.81} & {83.12} & \underline{46.16} & {68.86} & {51.33} & {53.75} & {70.23} \\
		% OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} & - & - & - & - & - & - & - & - & 96.3\\
		Holo2-8B*~\citep{hai2025holo2modelfamily}                         & 71.4 & 85.8 & 77.9 & 76.8 & 34.0 & 63.1 & 0.0 & 30.2 & 56.4 \\
		Holo2-30B-A3B*~\citep{hai2025holo2modelfamily}                    & 78.1 & 89.7 & 81.0 & 81.8 & 32.2 & 68.7 & 0.0 & 31.0 & 59.5 \\
		Step-GUI-4B*~\citep{yan2025step}                      & 73.9 & 81.8 & 77.9 & 77.0 & 26.1 & 59.0 & 0.0 & 25.9 & 54.6 \\
		% Step-GUI-8B~\citep{yan2025step}                      & - & -  & - & - & - & - & - & - & 95.1 \\
		MAI-UI-2B*~\citep{zhou2025mai}                        & 72.8 & 87.1 & 76.6 & 77.4 & 27.3 & 62.3 & 0.0 & 27.3 & 55.4 \\
		MAI-UI-8B*~\citep{zhou2025mai}                        & 81.3 & 90.8 & 84.5 & 84.5 & \textbf{55.4} & \underline{69.1} & 0.0 & 40.5 & 65.2 \\
		% MAI-UI-32B~\citep{zhou2025mai}                       & - & - & - & - & - & - & - & - & {96.5}\\
		\midrule
		\rowcolor{gray!15}
		\multicolumn{10}{l}{\textit{Ours}} \\
		UI-Venus-1.5-2B                       & 79.4 & 85.8 & 80.9 & 81.4 & 22.0 & 57.3 & \textbf{76.3} & 49.2 & 67.3 \\
		UI-Venus-1.5-8B                       & \underline{84.2} & \underline{93.1} & \underline{84.9} & \underline{86.6} & 38.1 & \textbf{70.1} & 61.6 & \underline{54.2} & \underline{72.3} \\
		UI-Venus-1.5-30B-A3B                      & \textbf{85.1} & \textbf{93.2} & \textbf{86.4} & \textbf{87.5} & 41.8 & 68.1 & \underline{73.1} & \textbf{59.0} & \textbf{75.0} \\
		\bottomrule
	\end{tabular*}
	\vspace{-0.4em}
	\caption{Performance comparison on \textbf{VenusBench-GD}. For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and \underline{underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.}
	\label{tab:venusbench-gd}
\end{table}


==> tables/venusbench_mobile.tex <==

% \begin{table*}[t]
% 	\footnotesize
%   \centering
%   \caption{
% Performance comparison on \textbf{VenusBench-Mobile}.
%  For each benchmark, the best and second-best performing models are indicated in \textbf{bold} and {underlined}, respectively. Asterisk (*) indicates results that may require verification with original sources.
%   }
%   \label{tab:mainresults}
%   \resizebox{\textwidth}{!}{
%   \begin{tabular}{lccccccccc|c}
%     \toprule
%     Agent & FA & CF & VA & MR & GSA & GUIM & HGB & NR & BC & Total \\
%     \midrule
%     \rowcolor{gray!15}
%     \multicolumn{11}{l}{\textit{General VLMs}} \\
%     Qwen3-VL-8B~\cite{Qwen3-VL}         & 18.2 & 4.6 & 18.8 & 0.0 & 0.0 & 0.0 & 0.0 & 6.3 & 10.0 & 6.7 \\
%     Qwen3-VL-30B-A3B~\cite{Qwen3-VL}    & 22.7 & 4.6 & 18.8 & 0.0 & 0.0 & 0.0 & 5.9 & 6.3 & 10.0 & 8.7 \\
%     \midrule
%     \rowcolor{gray!15}
%     \multicolumn{11}{l}{\textit{GUI-specific Models}} \\
%         UI-Venus-7B~\cite{gu2025ui}         & 13.6 & 4.6 & 25.0 & 0.0 & 10.0 & 0.0 & 0.0 & 18.8 & 0.0 & 8.1 \\
%     UI-Venus-72B~\cite{gu2025ui}        & 22.7 & 4.6 & 12.5 & 0.0 & 10.0 & 0.0 & 17.7 & 50.0 & 0.0 & 15.4 \\
%     GUI-Owl-7B~\cite{ye2025mobile}          & 13.6 & 0.0 & 18.8 & 0.0 & 0.0 & 11.1 & 2.9 & 12.5 & 0.0 & 6.7 \\
%     MA3{\small(GUI-Owl-7B)}~\cite{ye2025mobile} & 18.2 & 9.1 & 6.3 & 0.0 & 0.0 & 0.0 & 11.8 & 31.3 & 20.0 & 12.1 \\
%     MAI-UI-2B~\cite{zhou2025mai}           & 9.1 & 0.0 & 18.8 & 0.0 & 0.0 & 0.0 & 0.0 & 25.0 & 10.0 & 6.7 \\
%     MAI-UI-8B~\cite{zhou2025mai}           & 9.1 & 13.6 & 25.0 & 0.0 & 10.0 & 11.1 & 5.9 & 31.3 & 10.0 & 12.8 \\
%     \midrule
%     \rowcolor{gray!15}\multicolumn{11}{l}{\textit{Ours}} \\
%     UI-Venus-1.5-2B     & 22.7 & 0.0 & 12.5 & 0.0 & 10.0 & 11.1 & 2.9 & 18.8 & 0.0 & 8.7 \\
%     UI-Venus-1.5-8B     & 22.7 & 0.0 & 25.0 & 0.0 & 0.0 & 22.2 & 8.8 & 50.0 & 20.0 & 16.1 \\
%     UI-Venus-1.5-30B-A3B& 40.9 & 0.0 & 37.5 & 10.0 & 20.0 & 22.2 & 14.7 & 43.8 & 0.0 & 21.5 \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table*}


\begin{table*}[t]
	\footnotesize
  \centering
  \caption{Performance comparison on \textbf{VenusBench-Mobile}. The best performing model is indicated in \textbf{bold}.}
  \label{tab:mainresults}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lccccccccc|c}
    \toprule
    \textbf{Agent} & \textbf{FA} & \textbf{CF} & \textbf{VA} & \textbf{MR} & \textbf{GSA} & \textbf{GUIM} & \textbf{HGB} & \textbf{NR} & \textbf{BC} & \textbf{Total} \\
    \midrule
    \rowcolor{gray!15}
    \multicolumn{11}{l}{\textit{General VLMs}} \\
    Qwen3-VL-8B~\cite{Qwen3-VL}         & 18.2 & 4.6 & 18.8 & 0.0 & 0.0 & 0.0 & 0.0 & 6.3 & {10.0} & 6.7 \\
    Qwen3-VL-30B-A3B~\cite{Qwen3-VL}    & {22.7} & 4.6 & 18.8 & 0.0 & 0.0 & 0.0 & 5.9 & 6.3 & {10.0} & 8.7 \\
    \midrule
    \rowcolor{gray!15}
    \multicolumn{11}{l}{\textit{GUI-specific Models}} \\
    UI-Venus-7B~\cite{gu2025ui}         & 13.6 & 4.6 & {25.0} & 0.0 & {10.0} & 0.0 & 0.0 & 18.8 & 0.0 & 8.1 \\
    UI-Venus-72B~\cite{gu2025ui}        & {22.7} & 4.6 & 12.5 & 0.0 & {10.0} & 0.0 & \textbf{17.7} & \textbf{50.0} & 0.0 & {15.4} \\
    GUI-Owl-7B~\cite{ye2025mobile}          & 13.6 & 0.0 & 18.8 & 0.0 & 0.0 & {11.1} & {2.9} & 12.5 & 0.0 & 6.7 \\
    MA3{\small(GUI-Owl-7B)}~\cite{ye2025mobile} & 18.2 & {9.1} & 6.3 & 0.0 & 0.0 & 0.0 & {11.8} & {31.3} & \textbf{20.0} & {12.1} \\
    MAI-UI-2B~\cite{zhou2025mai}           & 9.1 & 0.0 & 18.8 & 0.0 & 0.0 & 0.0 & 0.0 & 25.0 & {10.0} & 6.7 \\
    MAI-UI-8B~\cite{zhou2025mai}           & 9.1 & \textbf{13.6} & {25.0} & 0.0 & {10.0} & {11.1} & 5.9 & {31.3} & {10.0} & {12.8} \\
    \midrule
    \rowcolor{gray!15}\multicolumn{11}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B     & {22.7} & 0.0 & 12.5 & 0.0 & {10.0} & {11.1} & {2.9} & 18.8 & 0.0 & 8.7 \\
    UI-Venus-1.5-8B     & {22.7} & 0.0 & {25.0} & 0.0 & 0.0 & \textbf{22.2} & 8.8 & \textbf{50.0} & \textbf{20.0} & {16.1} \\
    UI-Venus-1.5-30B-A3B& \textbf{40.9} & 0.0 & \textbf{37.5} & \textbf{10.0} & \textbf{20.0} & \textbf{22.2} & {14.7} & {43.8} & 0.0 & \textbf{21.5} \\
    \bottomrule
  \end{tabular}
  }
\end{table*}


==> tables/webvoyager_exp.tex <==


% \begin{table}[ht]
%     \centering
%     \footnotesize
%     %\setlength{\tabcolsep}{0pt}
%     \begin{tabular}{lcc}
%     \toprule
%     \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
%     \midrule
%     \rowcolor{gray!15}
%     \multicolumn{3}{l}{\textit{General VLMs}} \\
%     Qwen3-VL-2B~\citep{Qwen3-VL}                      &  2B    &       35.21                     \\ 
%     Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    &        45.26                  \\ 
%     Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &    47.55                      \\ 
%     Gemini-2.5-Pro~\citep{comanici2025gemini}  & -   &                      \\ 
%     Seed1.8~\citep{seed1.8}  & -   &                      \\ 
%     \midrule
%     \rowcolor{gray!15}
%     \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
%     ScaleCUA-3B~\citep{}                      &  3B         &                           \\ 
%     UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                      &  7B     &                     \\ 
%     GUI-Owl-7B ~\citep{}                      &  7B     &                      \\ 
%     UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui}               &   72B    &   \\
%     Holo2-4B~\citep{hai2025holo2modelfamily}                      &  8B     &      80.2                \\ 
%     Holo2-8B~\citep{hai2025holo2modelfamily}                     &  8B     &      80.2                \\ 
%     Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                   &  30B     &    83.0                  \\ 
%     \midrule
%     \rowcolor{gray!15}
%     \multicolumn{3}{l}{\textit{Ours}} \\
%     UI-Venus-1.5-2B              &  2B &             \\ 
%     UI-Venus-1.5-8B              &  8B &             \\ 
%     UI-Venus-1.5-30B-A3B              &  30B     &                \\ 
    
%     \bottomrule
%     \end{tabular}
%     \vspace{0.4em}
%     \caption{Performance comparison on \textbf{WebVoyager} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
%     \label{tab:webvoyager}
% \end{table}


\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Model} & \textbf{Params.} & \textbf{Success Rate} \\
\midrule

\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{General VLMs}} \\
Qwen3-VL-8B~\citep{Qwen3-VL} & 8B  &  \\
Qwen3-VL-32B~\citep{Qwen3-VL} & 32B  &  \\
Qwen3.5-9B~\citep{qwen3.5} & 9B  & 46.9 \\
Qwen3.6-27B~\citep{qwen3.5} & 27B  & 84.3 \\
Gemini-2.5-Pro~\citep{comanici2025gemini} & -- & -- \\
Seed2.0~\citep{seed2} & -- & 85.1 \\
Glm-5v-turbo \citep{hong2026glm} & -- & 88.5 \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{GUI-specific Models}} \\
UI-TARS-1.5~\citep{ui-tars-15-seed} & & 84.8 \\
UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui} & 72B & -- \\
Holo2-4B~\citep{hai2025holo2modelfamily} & 4B  & 80.2 \\
Holo2-8B~\citep{hai2025holo2modelfamily} & 8B  & 80.2 \\
Holo2-30B-A3B~\citep{hai2025holo2modelfamily} & 30B & 83.0 \\
Fara~\citep{fara7b2025} & 7B & 73.5 \\
Fara-1.5~\citep{awadallah2026fara} & 9B & 86.6 \\
GUI-Owl-1.5-8B-Instruct \cite{xu2026mobile} & 8B & 69.9 \\
GUI-Owl-1.5-8B-Thinking \cite{xu2026mobile} & 8B & 78.1 \\
GUI-Owl-1.5-32B-Thinking \cite{xu2026mobile} & 32B & 82.1 \\
UI-Venus-1.5-2B \cite{team2026ui} & 2B & 56.4 \\
UI-Venus-1.5-8B \cite{team2026ui} & 8B & 70.8 \\
UI-Venus-1.5-30B-A3B \cite{team2026ui} & 30B & 76.0 \\

\midrule
\rowcolor{gray!15}
\multicolumn{3}{@{}l}{\textit{Ours}} \\
UI-Venus-2-4B
    & 4B  & -- \\
UI-Venus-2-9B
    & 9B  & -- \\

@article{hong2026glm,
  title={Glm-5v-turbo: Toward a native foundation model for multimodal agents},
  author={Hong, Wenyi and Gu, Xiaotao and Pan, Ziyang and Yang, Zhen and Wang, Yuting and Wang, Yue and Yue, Yuanchang and Wang, Yu and Wang, Yanling and Wang, Yan and others},
  journal={arXiv preprint arXiv:2604.26752},
  year={2026}
}

GLM-5V-Turbo \cite{hong2026glm}
GUI-Owl-

\bottomrule
\end{tabular}
\vspace{0.3em}
\caption{
Performance comparison on \textbf{WebVoyager}.
UI-Venus-1.5 achieves state-of-the-art performance across model scales.
}
\label{tab:webvoyager}
\end{table}
